AirIndex: Versatile Index Tuning Through Data and Storage

The end-to-end lookup latency of a hierarchical index -- such as a B-tree or a learned index -- is determined by its structure such as the number of layers, the kinds of branching functions appearing in each layer, the amount of data we must fetch from layers, etc. Our primary observation is that by optimizing those structural parameters (or designs) specifically to a target system's I/O characteristics (e.g., latency, bandwidth), we can offer a faster lookup compared to the ones that are not optimized. Can we develop a systematic method for finding those optimal design parameters? Ideally, the method must have the potential to generate almost any existing index or a novel combination of them for the fastest possible lookup. In this work, we present new data and an I/O-aware index builder (called AirIndex) that can find high-speed hierarchical index designs in a principled way. Specifically, AirIndex minimizes an objective function expressing the end-to-end latency in terms of various designs -- the number of layers, types of layers, and more -- for given data and a storage profile, using a graph-based optimization method purpose-built to address the computational challenges rising from the inter-dependencies among index layers and the exponentially many candidate parameters in a large search space. Our empirical studies confirm that AirIndex can find optimal index designs, build optimal indexes within the times comparable to existing methods, and deliver up to 4.1x faster lookup than a lightweight B-tree library (LMDB), 3.3x--46.3x faster than state-of-the-art learned indexes (RMI/CDFShop, PGM-Index, ALEX/APEX, PLEX), and 2.0 faster than Data Calculator's suggestion on various dataset and storage settings.

==> figures/background/motivation.tex <==
\begin{figure*}

\tikzset{
mynode/.style={
    draw=black,thick,font=\scriptsize\sf,
    minimum height=3mm,minimum width=4mm,
    inner ysep=0.4mm,
},
mylarge/.style={
    mynode,minimum width=16mm,
},
mylayer/.style={
    draw=gray!50!white,ultra thick,rounded corners=1mm,
    inner ysep=0.5mm,inner xsep=1mm
}
}


\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture} 

\def\h{0.6}
\def\d{0.05}

\node[mynode] (L1) at (0,0) {};

\node[mynode] (L21) at ($(L1)+(-0.8,-\h)$) {};
\node[mynode,anchor=west] (L22) at ($(L21.east)+(\d,0)$) {};
\node[mynode,anchor=west,draw opacity=0,font=\Large\bf] (L23) at ($(L22.east)+(\d,0)$) {$\cdots$};
\node[mynode,anchor=west] (L24) at ($(L23.east)+(\d,0)$) {};

\node[mynode] (L31) at ($(L21)+(-0.65,-\h)$) {};
\node[mynode,anchor=west] (L32) at ($(L31.east)+(\d,0)$) {};
\node[mynode,anchor=west] (L33) at ($(L32.east)+(\d,0)$) {};
\node[mynode,anchor=west,draw opacity=0,font=\Large\bf] (L34) at ($(L33.east)+(\d,0)$) {$\cdots$};
\node[mynode,anchor=west] (L35) at ($(L34.east)+(\d,0)$) {};
\node[mynode,anchor=west] (L36) at ($(L35.east)+(\d,0)$) {};

\node[mynode,minimum width=50mm] (D) at ($(L31)!0.5!(L36) + (0,-\h)$) {Data Layer};

% Layers
\node[mylayer,fit={(L21.north west) (L24.south east)}] {};

\node[mylayer,fit={(L31.north west) (L36.south east)}] {};

% Arrows
\draw[->,draw=black,ultra thick] (L1) -- (L22);
\draw[->,draw=black,ultra thick] (L22) -- (L33);
\draw[->,draw=black,ultra thick] (L33) -- ($(D.north)+(-1,0)$);

\end{tikzpicture}
\caption{B+ tree}
\label{fig:motivation:a}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\centering
\begin{tikzpicture} 

\def\h{0.6}
\def\d{0.05}

\node[mynode] (L1) at (0,0) {};

\node[mynode,minimum width=35mm] (L21) at ($(L1)+(0,-\h)$) {};

\node[mynode,minimum width=50mm] (D) at ($(L21)+(0,-\h)$) {Data Layer};

\end{tikzpicture}
\caption{Learned Index}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
\caption{\system}
\end{subfigure}

\vspace{-2mm}
\caption{A need to learn from storage performance as well as data distributions. \todo{remove if not enough time}}
\end{figure*}


==> figures/background/structures/2_band.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.75]
%uncomment if require: \path (0,122); %set diagram left start at 0, and has height of 122

%Shape: Rectangle [id:dp7196748290967514] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (10,0) -- (80,0) -- (80,20.6) -- (10,20.6) -- cycle ;
%Shape: Rectangle [id:dp3856860319686912] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (5,50) -- (85,50) -- (85,70.2) -- (5,70.2) -- cycle ;
%Shape: Rectangle [id:dp7000162378600776] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]  (0,99.8) -- (90,99.8) -- (90,120) -- (0,120) -- cycle ;
%Straight Lines [id:da8678501685913436] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (40,20) -- (21.66,47.5) ;
\draw [shift={(20,50)}, rotate = 303.69] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da7442290269578888] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (40,20) -- (40,47) ;
\draw [shift={(40,50)}, rotate = 270] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da7327825732357917] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (40,70) -- (21.66,97.5) ;
\draw [shift={(20,100)}, rotate = 303.69] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da04599539286426968] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (40,70) -- (40,97) ;
\draw [shift={(40,100)}, rotate = 270] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;

% Text Node
\draw (45,10.3) node [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  [align=left] {{\scriptsize \textcolor[rgb]{0.29,0.56,0.89}{PWL} \textbf{1KB}}};
% Text Node
\draw (45,60.1) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {{\scriptsize \textcolor[rgb]{0.29,0.56,0.89}{PWL}}};
% Text Node
\draw (45,109.9) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {{\scriptsize Data Layer}};
% Text Node
\draw (59,35) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {{\scriptsize \textbf{16KB}}};
% Text Node
\draw (59,85) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {{\scriptsize \textbf{16KB}}};


\end{tikzpicture}

==> figures/data/storage_variability.tex <==
\pgfplotstableread{
%% 0.0 0.0 0.012 0.12 1.2000000000000002 12.0 120.0 1200.0 12000.0 MB/s
rellat lat la lb lc ld le lf lg
0.001000 50000.000000 121.589694 118.742583 96.226726 35.339914 6.510695 1.500084 1.000000
0.001259 62946.270590 121.505872 117.948083 91.252881 30.357126 5.613734 1.335373 1.000000
0.001585 79244.659623 121.400512 116.962901 85.679875 25.797391 4.844699 1.202143 1.000000
0.001995 99763.115748 121.268131 115.745852 79.565739 21.713341 4.160871 1.094766 1.000000
0.002512 125594.321575 121.101885 114.249327 73.011072 18.464694 3.563895 1.008477 1.000000
0.003162 158113.883008 120.893243 112.419612 66.155840 15.818576 3.051050 1.000000 1.000000
0.003981 199053.585277 120.631600 110.198057 59.169279 13.422336 2.616533 1.000000 1.000000
0.005012 250593.616814 120.303822 107.523454 52.234027 11.296233 2.252671 1.000000 1.000000
0.006310 315478.672240 119.893704 104.335988 46.196930 9.443720 1.950958 1.000000 1.000000
0.007943 397164.117362 119.381367 100.583029 40.658975 7.854926 1.702810 1.000000 1.000000
0.010000 500000.000000 118.742583 96.226726 35.339914 6.510695 1.500084 1.000000 1.000000
0.012589 629462.705897 117.948083 91.252881 30.357126 5.613734 1.335373 1.000000 1.000000
0.015849 792446.596231 116.962901 85.679875 25.797391 4.844699 1.202143 1.000000 1.000000
0.019953 997631.157484 115.745852 79.565739 21.713341 4.160871 1.094766 1.000000 1.000000
0.025119 1255943.215755 114.249327 73.011072 18.464694 3.563895 1.008477 1.000000 1.000000
0.031623 1581138.830084 112.419612 66.155840 15.818576 3.051050 1.000000 1.000000 1.000000
0.039811 1990535.852767 110.198057 59.169279 13.422336 2.616533 1.000000 1.000000 1.000000
0.050119 2505936.168136 107.523454 52.234027 11.296233 2.252671 1.000000 1.000000 1.000000
0.063096 3154786.722401 104.335988 46.196930 9.443720 1.950958 1.000000 1.000000 1.000000
0.079433 3971641.173621 100.583029 40.658975 7.854926 1.702810 1.000000 1.000000 1.000000
0.100000 5000000.000000 96.226726 35.339914 6.510695 1.500084 1.000000 1.000000 1.000000
0.125893 6294627.058971 91.252881 30.357126 5.613734 1.335373 1.000000 1.000000 1.000000
0.158489 7924465.962306 85.679875 25.797391 4.844699 1.202143 1.000000 1.000000 1.000000
0.199526 9976311.574844 79.565739 21.713341 4.160871 1.094766 1.000000 1.000000 1.000000
0.251189 12559432.157548 73.011072 18.464694 3.563895 1.008477 1.000000 1.000000 1.000000
0.316228 15811388.300842 66.155840 15.818576 3.051050 1.000000 1.000000 1.000000 1.000000
0.398107 19905358.527675 59.169279 13.422336 2.616533 1.000000 1.000000 1.000000 1.000000
0.501187 25059361.681364 52.234027 11.296233 2.252671 1.000000 1.000000 1.000000 1.000000
0.630957 31547867.224010 46.196930 9.443720 1.950958 1.000000 1.000000 1.000000 1.000000
0.794328 39716411.736214 40.658975 7.854926 1.702810 1.000000 1.000000 1.000000 1.000000
1.000000 50000000.000000 35.339914 6.510695 1.500084 1.000000 1.000000 1.000000 1.000000
1.258925 62946270.589708 30.357126 5.613734 1.335373 1.000000 1.000000 1.000000 1.000000
1.584893 79244659.623056 25.797391 4.844699 1.202143 1.000000 1.000000 1.000000 1.000000
1.995262 99763115.748444 21.713341 4.160871 1.094766 1.000000 1.000000 1.000000 1.000000
2.511886 125594321.575479 18.464694 3.563895 1.008477 1.000000 1.000000 1.000000 1.000000
3.162278 158113883.008419 15.818576 3.051050 1.000000 1.000000 1.000000 1.000000 1.085073
3.981072 199053585.276749 13.422336 2.616533 1.000000 1.000000 1.000000 1.000000 1.197763
5.011872 250593616.813636 11.296233 2.252671 1.000000 1.000000 1.000000 1.000000 1.305459
6.309573 315478672.240097 9.443720 1.950958 1.000000 1.000000 1.000000 1.000000 1.405869
7.943282 397164117.362141 7.854926 1.702810 1.000000 1.000000 1.000000 1.000000 1.497353
10.000000 500000000.000000 6.510695 1.500084 1.000000 1.000000 1.000000 1.000000 1.578969
12.589254 629462705.897083 5.613734 1.335373 1.000000 1.000000 1.000000 1.000000 1.650427
15.848932 792446596.230557 4.844699 1.202143 1.000000 1.000000 1.000000 1.000000 1.711969
19.952623 997631157.484439 4.160871 1.094766 1.000000 1.000000 1.000000 1.000000 1.764225
25.118864 1255943215.754791 3.563895 1.008477 1.000000 1.000000 1.000000 1.000000 1.808063
31.622777 1581138830.084190 3.051050 1.000000 1.000000 1.000000 1.000000 1.085073 1.844469
39.810717 1990535852.767485 2.616533 1.000000 1.000000 1.000000 1.000000 1.197763 1.874449
50.118723 2505936168.136363 2.252671 1.000000 1.000000 1.000000 1.000000 1.305459 1.898967
63.095734 3154786722.400965 1.950958 1.000000 1.000000 1.000000 1.000000 1.405869 1.918904
79.432823 3971641173.621410 1.702810 1.000000 1.000000 1.000000 1.000000 1.497353 1.935041
100.000000 5000000000.000000 1.500084 1.000000 1.000000 1.000000 1.000000 1.578969 1.948055
125.892541 6294627058.970831 1.335373 1.000000 1.000000 1.000000 1.000000 1.650427 1.958517
158.489319 7924465962.305571 1.202143 1.000000 1.000000 1.000000 1.000000 1.711969 1.966907
199.526231 9976311574.844393 1.094766 1.000000 1.000000 1.000000 1.000000 1.764225 1.973624
251.188643 12559432157.547911 1.008477 1.000000 1.000000 1.000000 1.000000 1.808063 1.978992
316.227766 15811388300.841898 1.000000 1.000000 1.000000 1.000000 1.085073 1.844469 1.983276
398.107171 19905358527.674847 1.000000 1.000000 1.000000 1.000000 1.197763 1.874449 1.986693
501.187234 25059361681.363625 1.000000 1.000000 1.000000 1.000000 1.305459 1.898967 1.989415
630.957344 31547867224.009651 1.000000 1.000000 1.000000 1.000000 1.405869 1.918904 1.991583
794.328235 39716411736.214111 1.000000 1.000000 1.000000 1.000000 1.497353 1.935041 1.993309
1000.000000 50000000000.000000 1.000000 1.000000 1.000000 1.000000 1.578969 1.948055 1.994681
}\nfsvariability

\pgfplotstableread{
%% 0.0 0.0 0.17500000000000002 1.75 17.5 175.0 1750.0 17500.0 175000.0 MB/s
rellat lat la lb lc ld le lf lg
0.001000 250.000000 6.856450 6.845298 6.735888 5.818784 2.729307 1.089387 1.000000
0.001259 314.731353 6.856129 6.842097 6.705106 5.602876 2.456692 1.027970 1.000000
0.001585 396.223298 6.855724 6.838071 6.666784 5.354778 2.198971 1.000000 1.000000
0.001995 498.815579 6.855215 6.833010 6.619208 5.074765 1.961119 1.000000 1.000000
0.002512 627.971608 6.854574 6.826651 6.560346 4.765069 1.746428 1.000000 1.000000
0.003162 790.569415 6.853767 6.818663 6.487834 4.430125 1.564823 1.000000 1.000000
0.003981 995.267926 6.852752 6.808635 6.398978 4.076529 1.447772 1.000000 1.038166
0.005012 1252.968084 6.851474 6.796056 6.290796 3.712643 1.340908 1.000000 1.107317
0.006310 1577.393361 6.849866 6.780291 6.160118 3.347870 1.245394 1.000000 1.169598
0.007943 1985.820587 6.847843 6.760557 6.003758 3.010434 1.161631 1.000000 1.224589
0.010000 2500.000000 6.845298 6.735888 5.818784 2.729307 1.089387 1.000000 1.272300
0.012589 3147.313529 6.842097 6.705106 5.602876 2.456692 1.027970 1.000000 1.313068
0.015849 3962.232981 6.838071 6.666784 5.354778 2.198971 1.000000 1.000000 1.347452
0.019953 4988.155787 6.833010 6.619208 5.074765 1.961119 1.000000 1.000000 1.376135
0.025119 6279.716079 6.826651 6.560346 4.765069 1.746428 1.000000 1.000000 1.399843
0.031623 7905.694150 6.818663 6.487834 4.430125 1.564823 1.000000 1.000000 1.419291
0.039811 9952.679264 6.808635 6.398978 4.076529 1.447772 1.000000 1.038166 1.435145
0.050119 12529.680841 6.796056 6.290796 3.712643 1.340908 1.000000 1.107317 1.448003
0.063096 15773.933612 6.780291 6.160118 3.347870 1.245394 1.000000 1.169598 1.458389
0.079433 19858.205868 6.760557 6.003758 3.010434 1.161631 1.000000 1.224589 1.466751
0.100000 25000.000000 6.735888 5.818784 2.729307 1.089387 1.000000 1.272300 1.473463
0.125893 31473.135295 6.705106 5.602876 2.456692 1.027970 1.000000 1.313068 1.478841
0.158489 39622.329812 6.666784 5.354778 2.198971 1.000000 1.000000 1.347452 1.483142
0.199526 49881.557874 6.619208 5.074765 1.961119 1.000000 1.000000 1.376135 1.486577
0.251189 62797.160788 6.560346 4.765069 1.746428 1.000000 1.000000 1.399843 1.489317
0.316228 79056.941504 6.487834 4.430125 1.564823 1.000000 1.000000 1.419291 1.491502
0.398107 99526.792638 6.398978 4.076529 1.447772 1.000000 1.038166 1.435145 1.493241
0.501187 125296.808407 6.290796 3.712643 1.340908 1.000000 1.107317 1.448003 1.494626
0.630957 157739.336120 6.160118 3.347870 1.245394 1.000000 1.169598 1.458389 1.495728
0.794328 198582.058681 6.003758 3.010434 1.161631 1.000000 1.224589 1.466751 1.496605
1.000000 250000.000000 5.818784 2.729307 1.089387 1.000000 1.272300 1.473463 1.497302
1.258925 314731.352949 5.602876 2.456692 1.027970 1.000000 1.313068 1.478841 1.497856
1.584893 396223.298115 5.354778 2.198971 1.000000 1.000000 1.347452 1.483142 1.498296
1.995262 498815.578742 5.074765 1.961119 1.000000 1.000000 1.376135 1.486577 1.498646
2.511886 627971.607877 4.765069 1.746428 1.000000 1.000000 1.399843 1.489317 1.498925
3.162278 790569.415042 4.430125 1.564823 1.000000 1.000000 1.419291 1.491502 1.499146
3.981072 995267.926384 4.076529 1.447772 1.000000 1.038166 1.435145 1.493241 1.499321
5.011872 1252968.084068 3.712643 1.340908 1.000000 1.107317 1.448003 1.494626 1.499461
6.309573 1577393.361200 3.347870 1.245394 1.000000 1.169598 1.458389 1.495728 1.499572
7.943282 1985820.586811 3.010434 1.161631 1.000000 1.224589 1.466751 1.496605 1.499660
10.000000 2500000.000000 2.729307 1.089387 1.000000 1.272300 1.473463 1.497302 1.499730
12.589254 3147313.529485 2.456692 1.027970 1.000000 1.313068 1.478841 1.497856 1.499785
15.848932 3962232.981153 2.198971 1.000000 1.000000 1.347452 1.483142 1.498296 1.499829
19.952623 4988155.787422 1.961119 1.000000 1.000000 1.376135 1.486577 1.498646 1.499865
25.118864 6279716.078774 1.746428 1.000000 1.000000 1.399843 1.489317 1.498925 1.499892
31.622777 7905694.150421 1.564823 1.000000 1.000000 1.419291 1.491502 1.499146 1.499915
39.810717 9952679.263837 1.447772 1.000000 1.038166 1.435145 1.493241 1.499321 1.563616
50.118723 12529680.840682 1.340908 1.000000 1.107317 1.448003 1.494626 1.499461 1.734411
63.095734 15773933.612005 1.245394 1.000000 1.169598 1.458389 1.495728 1.499572 1.899195
79.432823 19858205.868107 1.161631 1.000000 1.224589 1.466751 1.496605 1.499660 2.054224
100.000000 25000000.000000 1.089387 1.000000 1.272300 1.473463 1.497302 1.499730 2.196654
125.892541 31473135.294854 1.027970 1.000000 1.313068 1.478841 1.497856 1.499785 2.324687
158.489319 39622329.811528 1.000000 1.000000 1.347452 1.483142 1.498296 1.499829 2.437539
199.526231 49881557.874222 1.000000 1.000000 1.376135 1.486577 1.498646 1.499865 2.535302
251.188643 62797160.787740 1.000000 1.000000 1.399843 1.489317 1.498925 1.499892 2.618731
316.227766 79056941.504209 1.000000 1.000000 1.419291 1.491502 1.499146 1.499915 2.689018
398.107171 99526792.638374 1.000000 1.038166 1.435145 1.493241 1.499321 1.563616 2.747597
501.187234 125296808.406818 1.000000 1.107317 1.448003 1.494626 1.499461 1.734411 2.795979
630.957344 157739336.120048 1.000000 1.169598 1.458389 1.495728 1.499572 1.899195 2.835641
794.328235 198582058.681071 1.000000 1.224589 1.466751 1.496605 1.499660 2.054224 2.867957
1000.000000 250000000.000000 1.000000 1.272300 1.473463 1.497302 1.499730 2.196654 2.894157
}\ssdvariability

==> figures/dummy.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
      width=0.8\linewidth,
      axis lines=middle,
      grid,
      ymin=0,
      ymax=11,
      ytick={0,...,10},
      xmin=6,
      xmax=23,
      xtick={7,...,22},
      xticklabel={\pgfmathprintnumber{\tick}:00},
      xticklabel style={rotate=45,anchor=north east}]
    
        \addplot[draw=none] coordinates {(1,1)};
    \end{axis}
    \end{tikzpicture}
    
    \caption{\tofix{Dummy Empty Plot}}
    \label{fig:dummy_line}
    \vspace{-3mm}
\end{figure}

==> figures/dummy_line.tex <==
\begin{figure}[t]
    \centering
    \pgfplotstableread{
    dataset psql rocksdb rmi pwl
        1.00  1742.46 1606.44 260.24  147.62
        2.00  953.87  808.43  178.13  97.59
        4.00  501.46  409.41  130.16  60.29
        8.00  273.82  209.99  111.29  44.21
        16.00 158.26  110.21  97.19 35.22
        32.00 98.98 60.21 91.47 26.52
        64.00 68.86 35.21 87.22 20.86
        128.00  52.38 22.74 83.63 17.33
        256.00  43.87 16.51 81.84 14.83
        512.00  39.02 13.60 78.06 13.38
        1000.00 36.32 12.16 73.48 12.55
        2000.00 33.49 11.50 67.77 11.76
        % 3000.00 31.58 11.26 62.62 11.15
        4000.00 30.30 11.14 58.94 10.53
        % 5000.00 29.35 11.05 55.65 10.06
        % 6000.00 28.53 10.98 52.73 9.63
        % 7000.00 28.00 10.93 50.55 9.26
        8000.00 27.59 10.90 48.27 8.89
        % 9000.00 27.46 10.86 46.25 8.56
        % 10000.00  28.02 10.83 44.59 8.29
        % 11000.00  28.40 10.80 42.94 8.00
        % 12000.00  28.53 10.79 41.61 7.75
        % 13000.00  28.59 10.77 40.18 7.50
        % 14000.00  28.58 10.76 38.80 7.26
        % 15000.00  28.57 10.74 37.63 7.04
        16000.00  28.59 10.73 36.50 6.84
        % 17000.00  28.72 10.71 35.41 6.65
        % 18000.00  28.98 10.69 34.35 6.45
        % 19000.00  28.94 10.68 33.42 6.28
        % 20000.00  28.89 10.66 32.53 6.11
        % 21000.00  28.83 10.65 31.76 5.95
        % 22000.00  28.80 10.64 30.94 5.79
        % 23000.00  28.76 10.63 30.15 5.64
        % 24000.00  28.71 10.61 29.42 5.50
        % 25000.00  28.65 10.60 28.70 5.36
        % 26000.00  28.60 10.59 27.99 5.22
        % 27000.00  28.54 10.57 27.33 5.09
        % 28000.00  28.49 10.56 26.71 4.96
        % 29000.00  28.43 10.54 26.12 4.84
        % 30000.00  28.39 10.53 25.54 4.73
        % 31000.00  28.35 10.52 25.02 4.62
        32000.00  28.33 10.51 24.52 4.52
        % 33000.00  28.30 10.49 24.01 4.41
        % 34000.00  28.28 10.48 23.49 4.32
        % 35000.00  28.25 10.47 23.02 4.22
        % 36000.00  28.23 10.47 22.58 4.14
        % 37000.00  28.21 10.46 22.19 4.05
        % 38000.00  28.19 10.45 21.79 3.97
        % 39000.00  28.17 10.44 21.40 3.89
        % 40000.00  28.14 10.43 21.01 3.81
        % 41000.00  28.10 10.42 20.65 3.73
        % 42000.00  28.06 10.40 20.29 3.66
        % 43000.00  28.04 10.39 19.95 3.59
        % 44000.00  28.00 10.38 19.61 3.52
        % 45000.00  27.96 10.37 19.28 3.46
        % 46000.00  27.93 10.36 18.98 3.40
        % 47000.00  27.90 10.35 18.68 3.34
        % 48000.00  27.87 10.34 18.42 3.28
        % 49000.00  27.84 10.33 18.15 3.23
        % 50000.00  27.82 10.32 17.86 3.17
        % 51000.00  27.79 10.31 17.59 3.12
        % 52000.00  27.76 10.30 17.33 3.07
        % 53000.00  27.73 10.29 17.07 3.02
        % 54000.00  27.70 10.28 16.82 2.97
        % 55000.00  27.66 10.27 16.58 2.92
        % 56000.00  27.62 10.26 16.35 2.88
        % 57000.00  27.58 10.25 16.12 2.83
        % 58000.00  27.55 10.24 15.90 2.79
        % 59000.00  27.51 10.23 15.67 2.75
        % 60000.00  27.48 10.22 15.46 2.71
        % 61000.00  27.43 10.21 15.26 2.67
        % 62000.00  27.39 10.20 15.06 2.63
        % 63000.00  27.36 10.19 14.87 2.59
        64000.00  27.32 10.18 14.67 2.56
        % 65000.00  27.29 10.17 14.47 2.52
        % 66000.00  27.25 10.16 14.29 2.49
        % 67000.00  27.22 10.15 14.12 2.45
        % 68000.00  27.19 10.14 13.94 2.42
        % 69000.00  27.16 10.13 13.76 2.39
        70000.00  27.12 10.12 13.60 2.36
    }\ltqTable
    
    \begin{tikzpicture}
        \begin{axis}[
            height=45mm,
            width=1.0\linewidth,
            xmode=log,
            % xmin=1,
            % xmax=16,
            % ymin=0,
            % ymax=150,
            xlabel=Number of Queries $n$,
            xlabel near ticks,
            % ylabel=RMS Error,
            ymode=log,
            ylabel=Latency (ms/op),
            ylabel near ticks,
            ylabel style={align=center},
            % xtick={1, 4, 8, ..., 16},
            % xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
            % ytick={0, 30, 60, 90, 120, 150},
            % yticklabels={0\%, 30\%, 60\%, 90\%, 120\%, 150\%},
            % xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
            % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
            % extra y ticks={10, 20, 30, 40},
            % extra y tick style={yticklabels={}},
            % ylabel shift=-2pt,
            % xlabel shift=-2pt,
            legend style={
                % at={(0.5,1.55)},anchor=south,column sep=2pt,
                at={(0.99,0.97)},anchor=north east,column sep=2pt,
                % at={(0.42,-0.45)},anchor=north,column sep=2pt,
                % at={(1.02,1.0)},anchor=north west,column sep=2pt,
                draw=black,fill=white,line width=.5pt,
                font=\scriptsize,
                /tikz/every even column/.append style={column sep=5pt}
            },
            legend columns=2,
            colormap name=bright,
            every axis/.append style={font=\small},
            xmajorgrids,
            % xminorgrids,
            ymajorgrids,
            % yminorgrids,
            % minor grid style=lightgray,
            % nodes near coords,
            % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
        ]
        
        \addplot+[mark=x]
        table[x=dataset,y=psql] {\ltqTable};
        \addlegendentry{PostgreSQL}
        
        \addplot+[mark=o]
        table[x=dataset,y=rocksdb] {\ltqTable};
        \addlegendentry{RocksDB}
        
        \addplot+[mark=square]
        table[x=dataset,y=rmi] {\ltqTable};
        \addlegendentry{RMI}
        
        \addplot+[mark=diamond]
        table[x=dataset,y=pwl] {\ltqTable};
        \addlegendentry{\system}
        
        \end{axis}
    \end{tikzpicture}
        
    \caption{\tofix{Dummy Line Plot}}
    \label{fig:dummy_line}
    \vspace{-3mm}
\end{figure}


==> figures/examples/clipped_barplot.tex <==
\begin{figure}[t]
  \centering

\pgfplotsset{
    accfig/.style={
        width=0.75\linewidth,
        height=36mm,
        ybar,
        bar width=1.4mm,
        % xlabel=Corpus,
        xmin=0.5,
        xmax=3.5,
        xtick={1, 2, 3},
        xticklabels={
            \texttt{us-central1-c}, % \\(Iowa),
            \texttt{europe-west2-c}, % (London)},
            \texttt{asia-southeast1-b}, % (Singapore)}
        },
        % xticklabels={Iowa, London, Singapore},
        xticklabel style={rotate=10},
        ylabel near ticks,
        ylabel style={align=center},
        ymin=0,
        ymax=4400,
        ytick={0, 1000, ..., 4000},
        % yticklabels={0.1, 1, 10, 100, 1000},
        xticklabel style={yshift=2mm},
        xlabel style={yshift=0mm},
        % xtick style={draw=none},
        legend style={
            % at={(0.425,1.4)},anchor=south,column sep=2pt,
            % at={(0.99,0.97)},anchor=north east,column sep=2pt,
            % at={(0.42,-0.45)},anchor=north,column sep=2pt,
            at={(1.02,1.00)},anchor=north west,column sep=2pt,
            draw=black,fill=white,line width=.5pt,
            /tikz/every even column/.append style={column sep=5pt}
        },
        legend cell align={left},
        legend columns=1,
        area legend,
        clip=false,
        every axis/.append style={font=\scriptsize},
        % /pgfplots/ymode=log,
        /pgfplots/log origin=infty,
        minor tick num=1,
        minor grid style=lightgray,
        ymajorgrids,
        yminorgrids,
        % extra y ticks={10, 20, 30, 40},
        % extra y tick style={yticklabels={}},
        % ylabel shift=-2pt,
        % xlabel shift=-2pt,
        % yminorgrids,
        % ylabel shift=-4pt,
        % nodes near coords,
        % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
        },
    accfig/.belongs to family=/pgfplots/scale,
}
    \vspace{-9mm}

% \begin{subfigure}[b]{1.0\linewidth} \centering
    \begin{tikzpicture}

    \def\yclip{4800}
    \def\ycliptop{4800}
    \def\ycliplowerlower{4200}
    \def\ycliplower{4300}
    \def\yclipupper{4500}
    \def\yclipupperupper{4600}
    \newcommand\xmid[2]{#1 + #2}
    \newcommand\xlower[3]{\xmid{#1}{#2} - #3}
    \newcommand\xupper[3]{\xmid{#1}{#2} + #3}
    
    % x, x shift, x width, number
    \newcommand{\slabClipNumber}[4]{%
        \draw[fill=white,draw=white] (axis cs: \xlower{#1}{#2}{#3},\yclipupper) -- (axis cs: \xupper{#1}{#2}{#3},\yclipupperupper) -- (axis cs: \xupper{#1}{#2}{#3},\ycliplower) -- (axis cs: \xlower{#1}{#2}{#3},\ycliplowerlower) -- cycle;%
        \draw[draw=black] (axis cs: \xlower{#1}{#2}{#3},\yclipupper) -- (axis cs: \xupper{#1}{#2}{#3},\yclipupperupper);%
        \draw[draw=black] (axis cs: \xupper{#1}{#2}{#3},\ycliplower) -- (axis cs: \xlower{#1}{#2}{#3},\ycliplowerlower);%
        \node[anchor=west, rotate=90] at (axis cs: \xmid{#1}{#2},\ycliptop) {#4};%
    }
    
    \begin{axis}[accfig,
        % width=0.7\linewidth,
        ylabel=Search Latency (ms)]
    
    %%% Lucene
    \addplot[thick,draw=vintageblack,fill=vintageblack,
    postaction={
        pattern=north east lines,
        pattern color=white,
    }]
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % table[x=x,y=y] {
    x c y    y+
    % 1 0 254.8345557 {\yclip}
    1 0 254.8345557 3885.705658
    2 0 839.7534547 {\yclip}
    % 2 0 839.7534547 14117.8497
    3 0 2099.758349 {\yclip}
    % 3 0 2099.758349 37431.87928
    };
    % \slabClipNumber{1}{-0.17}{0.05}{3885};
    \slabClipNumber{2}{-0.25}{0.05}{14117};
    \slabClipNumber{3}{-0.25}{0.05}{37431};
    
    
    %%% Elasticsearch
    \addplot[thick,draw=vintageblack,fill=vintageblack]
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % table[x=x,y=y] {
    x c y    y+
    1 1 1655.994508 {\yclip}
    % 1 1 1655.994508 16474.48543
    2 1 1643.60251  {\yclip}
    % 2 1 1643.60251  16817.4931
    3 1 2128.250344 {\yclip}
    % 3 1 2128.250344 14688.09089
    };
    \slabClipNumber{1}{-0.125}{0.05}{16474};
    \slabClipNumber{2}{-0.125}{0.05}{16817};
    \slabClipNumber{3}{-0.125}{0.05}{14688};
    
    %%% SQLite
    \addplot[thick,draw=vintageblack!50,fill=vintageblack!50,]
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % table[x=x,y=y] {
    x c y    y+
    1 2 242.0121507 618.240363
    2 2 782.4309524 1628.206049
    % 3 2 1943.175542 {\yclip}
    3 2 1943.175542 4208.20374
    };
    % \slabClipNumber{3}{-0.044}{0.05}{4208};
    
    %%% Hash Table
    \addplot[thick,draw=vintageblack!50,fill=vintageblack!50,
    postaction={
        pattern=north east lines,
        pattern color=black,
    }]
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % table[x=x,y=y] {
    x c y    y+
    1 3 {\yclip} {\yclip}
    % 1 3 6781.6521 20881.15941
    2 3 {\yclip} {\yclip}
    % 2 3 7817.122712 50454.55853
    3 3 {\yclip} {\yclip}
    % 3 3 10545.37325 115839.6961
    };
    \slabClipNumber{1}{0.125}{0.05}{6781};
    \slabClipNumber{2}{0.125}{0.05}{7817};
    \slabClipNumber{3}{0.125}{0.05}{10545};
    
    % %%% MongoDB
    % \addplot[thick,draw=vintageblack,fill=white,]
    % plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    % table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % % table[x=x,y=y] {
    % x c y    y+
    % 1 5 68.47630172 279.557162
    % 2 5 456.9122215 1081.967206
    % 3 5 1032.354213 2142.152976
    % };
    
    %%% Airphant
    \addplot[thick,draw=vintageorange,fill=vintageorange,]
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % table[x=x,y=y] {
    x c y    y+
    1 4 175.3187697 477.434309
    2 4 414.801396  1070.681104
    3 4 1132.139502 2783.074737
    };
    
    
    
    
    %%% space
    % \addplot[thick,draw=vintageblack!50,fill=vintageblack!50,]
    % plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    % table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % % table[x=x,y=y] {
    % x c y    y+
    % 1 5 0.0 0.0
    % 2 5 0.0 0.0
    % 3 5 0.0 0.0
    % 4 5 0.0 0.0
    % 5 5 0.0 0.0
    % 6 5 0.0 0.0
    % 7 5 0.0 0.0
    % };
    
    % %%% Airphant on Filestore
    % \addplot[thick,draw=vintageorange,fill=vintageorange,]
    % plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    % table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % % table[x=x,y=y] {
    % x c y    y+
    % 1 6 85.34812786 269.702287
    % 2 6 379.3031376 767.54383
    % 3 6 861.1159632 2138.973016
    % };
    
    % \addplot[thick,draw=vintageorange!75,fill=vintageorange!75,]
    % % plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    % % table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % table[x=x,y=y] {
    % x c y    y+
    % 1 2 254.2812522 527.467323
    % 2 2 969.5631848 2641.066105
    % 3 2 405.6167708 1065.098625
    % 4 2 138.3479564 295.775295
    % 5 2 307.3329676 759.269984
    % 6 2 377.3756558 1322.527728
    % 7 2 348.9201379 825.136295
    % };
    
    % \addplot[thick,draw=vintageorange!50,fill=vintageorange!50,]
    % % plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    % % table[x=x,y=y,y error expr=\thisrowno{3}-\thisrowno{2}] {
    % table[x=x,y=y] {
    % x c y    y+
    % 1 1 274.5159123 621.050755
    % 2 1 637.6762959 1084.87594
    % 3 1 458.2496258 1573.012455
    % 4 1 184.7343866 1594.48116
    % 5 1 265.0517705 530.12317
    % 6 1 332.4198357 713.327716
    % 7 1 315.8083193 750.085184
    % };
    
    % \draw[fill=white,draw=white] (axis cs: 1.85,1825) -- (axis cs: 2.15,1875) -- (axis cs: 2.15,1775) -- (axis cs: 1.85,1725) -- cycle;
    % \draw[draw=black] (axis cs: 1.85,1825) -- (axis cs: 2.15,1875);
    % \draw[draw=black] (axis cs: 2.15,1775) -- (axis cs: 1.85,1725);
    
    % \draw[fill=white,draw=white] (axis cs: 2.85,1825) -- (axis cs: 3.15,1875) -- (axis cs: 3.15,1775) -- (axis cs: 2.85,1725) -- cycle;
    % \draw[draw=black] (axis cs: 2.85,1825) -- (axis cs: 3.15,1875);
    % \draw[draw=black] (axis cs: 3.15,1775) -- (axis cs: 2.85,1725);
    
    % \draw[fill=white,draw=white] (axis cs: 5.85,1825) -- (axis cs: 6.15,1875) -- (axis cs: 6.15,1775) -- (axis cs: 5.85,1725) -- cycle;
    % \draw[draw=black] (axis cs: 5.85,1825) -- (axis cs: 6.15,1875);
    % \draw[draw=black] (axis cs: 6.15,1775) -- (axis cs: 5.85,1725);
    
    % \draw[fill=white,draw=white] (axis cs: 6.85,1825) -- (axis cs: 7.15,1875) -- (axis cs: 7.15,1775) -- (axis cs: 6.85,1725) -- cycle;
    % \draw[draw=black] (axis cs: 6.85,1825) -- (axis cs: 7.15,1875);
    % \draw[draw=black] (axis cs: 7.15,1775) -- (axis cs: 6.85,1725);
    
    % \node[anchor=south] at (axis cs: 1,1900) {4072};
    % \node[anchor=south] at (axis cs: 1.5,1900) {2456};
    % \node[anchor=south] at (axis cs: 2.2,1900) {6683};
    % \node[anchor=south] at (axis cs: 3,1900) {3815};
    
    \addlegendentry{Lucene}
    \addlegendentry{Elasticsearch}
    \addlegendentry{SQLite}
    \addlegendentry{HashTable}
    % \addlegendentry{MongoDB$^{*}$}
    \addlegendentry{\system}
    % \addlegendentry{\system$^{*}$}
    % \addlegendentry{\system-0.01}
    % \addlegendentry{\system-0.0001}
      
    \end{axis}
    \end{tikzpicture}
    
    % \caption{Retrieval latency}
    % \label{fig:exp:e2e_selected:retrieval}
% \end{subfigure}

  \vspace{-2mm}
  \caption{End-to-end search latencies across regions.
  The \texttt{Windows} dataset was used. 
  Solid bars show averages; the upper error bars show 99th percentiles. 
%   Latencies over 6.6 seconds are truncated and labeled. 99 percentiles whose means are over the limit are omitted.
  }
  
  \label{fig:e2e_search_region}
  \vspace{-3mm}
\end{figure}
    


==> figures/examples/grouped_barplots.tex <==
\begin{figure}[t]
  \centering

\pgfplotsset{accfig/.style={
    width=1.0\linewidth,
    height=45mm,
    ybar,
    bar width=1.7mm,
    enlarge x limits=0.2,
    % xlabel=Corpus,
    % xmin=0.5,
    % xmax=7.5,
    symbolic x coords={books,fb,osm,wiki},
    xtick = data,
    % xtick={1, 2, 3, 4},
    xticklabels={\texttt{books}, \texttt{fb}, \texttt{osm}, \texttt{wiki}},
    % xticklabel style={rotate=18},
    ylabel={Initial Latency (ms)},
    ylabel near ticks,
    ylabel style={align=center},
    ymin=0,
    ymax=4000,
    ytick={0, 500, ..., 4000},
    % yticklabels={0.1, 1, 10, 100, 1000},
    % xticklabel style={yshift=2mm},
    % xlabel style={yshift=0mm},
    % xtick style={draw=none},
    legend style={
        % at={(0.5,1.55)},anchor=south,column sep=2pt,
        at={(0.99,0.97)},anchor=north east,column sep=2pt,
        % at={(0.42,-0.45)},anchor=north,column sep=2pt,
        % at={(1.02,1.0)},anchor=north west,column sep=2pt,
        draw=black,fill=white,line width=.5pt,
        font=\scriptsize,
        /tikz/every even column/.append style={column sep=5pt}
    },
    legend cell align={left},
    legend columns=1,
    colormap name=bright,
    area legend,
    % clip=false,
    every axis/.append style={font=\small},
    % ymode=log,
    minor tick num=1,
    minor grid style=lightgray,
    ymajorgrids,
    yminorgrids,
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    % ylabel shift=-2pt,
    % xlabel shift=-2pt,
    % yminorgrids,
    % ylabel shift=-4pt,
    % nodes near coords,
    % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
}}

\begin{tikzpicture}
    \begin{axis}[accfig]
    
    %%% PostgreSQL
    \addplot
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=dataset,y=l1] {
        method dataset l1 lc
        psql  books 2217.35 62.23
        psql  fb  1709.55 24.20
        % psql  lognormal 0.00 0.00
        % psql  normal  0.00 0.00
        psql  osm 2285.06 29.10
        % psql  uniform_dense 0.00 0.00
        % psql  uniform_sparse  0.00 0.00
        psql  wiki 1742.46 27.12
    };
    \addlegendentry{PostgreSQL}
    
    %%% RocksDB
    \addplot
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=dataset,y=l1] {
        method dataset l1 lc
        rocksdb books 3259.36 12.55
        rocksdb fb  1932.36 12.18
        % rocksdb lognormal 1916.30 13.83
        % rocksdb normal  1906.76 12.57
        rocksdb osm 3215.04 12.39
        % rocksdb uniform_dense 1779.73 11.30
        % rocksdb uniform_sparse  4197.87 5.76
        rocksdb wiki 1606.44 10.12
    };
    \addlegendentry{RocksDB}
    
    %%% RMI
    \addplot
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=dataset,y=l1] {
        method dataset l1 lc
        rmi books 285.10 44.71
        rmi fb  197.34 12.34
        % rmi lognormal 253.04 25.43
        % rmi normal  227.75 16.50
        rmi osm 270.50 57.41
        % rmi uniform_dense 196.02 16.66
        % rmi uniform_sparse  349.12 33.32
        rmi wiki 260.24 13.60
    };
    \addlegendentry{RMI}
    
    %%% AirIndex
    \addplot
    plot [error bars/.cd, y dir=plus,y explicit,error bar style={color=black}]
    table[x=dataset,y=l1] {
        method dataset l1 lc
        pwl books 141.17 8.96
        pwl fb  162.67 3.49
        % pwl lognormal 155.77 3.50
        % pwl normal  125.01 3.11
        pwl osm 203.00 9.02
        % pwl uniform_dense 158.67 3.32
        % pwl uniform_sparse  106.93 2.61
        pwl wiki 147.62 2.36
    };
    \addlegendentry{\system}
      
    \end{axis}
\end{tikzpicture}

  \vspace{-4mm}
  \caption{Initial lookup latency across SOSD datasets of different systems whose external memory is on Azure NFS.}
  \label{fig:latency_initial}
  \vspace{-4mm}
\end{figure}

==> figures/examples/multilines.tex <==
\begin{figure}[t]
    \centering
    \pgfplotstableread{
    dataset psql rocksdb rmi pwl
        1.00  1742.46 1606.44 260.24  147.62
        2.00  953.87  808.43  178.13  97.59
        4.00  501.46  409.41  130.16  60.29
        8.00  273.82  209.99  111.29  44.21
        16.00 158.26  110.21  97.19 35.22
        32.00 98.98 60.21 91.47 26.52
        64.00 68.86 35.21 87.22 20.86
        128.00  52.38 22.74 83.63 17.33
        256.00  43.87 16.51 81.84 14.83
        512.00  39.02 13.60 78.06 13.38
        1000.00 36.32 12.16 73.48 12.55
        2000.00 33.49 11.50 67.77 11.76
        % 3000.00 31.58 11.26 62.62 11.15
        4000.00 30.30 11.14 58.94 10.53
        % 5000.00 29.35 11.05 55.65 10.06
        % 6000.00 28.53 10.98 52.73 9.63
        % 7000.00 28.00 10.93 50.55 9.26
        8000.00 27.59 10.90 48.27 8.89
        % 9000.00 27.46 10.86 46.25 8.56
        % 10000.00  28.02 10.83 44.59 8.29
        % 11000.00  28.40 10.80 42.94 8.00
        % 12000.00  28.53 10.79 41.61 7.75
        % 13000.00  28.59 10.77 40.18 7.50
        % 14000.00  28.58 10.76 38.80 7.26
        % 15000.00  28.57 10.74 37.63 7.04
        16000.00  28.59 10.73 36.50 6.84
        % 17000.00  28.72 10.71 35.41 6.65
        % 18000.00  28.98 10.69 34.35 6.45
        % 19000.00  28.94 10.68 33.42 6.28
        % 20000.00  28.89 10.66 32.53 6.11
        % 21000.00  28.83 10.65 31.76 5.95
        % 22000.00  28.80 10.64 30.94 5.79
        % 23000.00  28.76 10.63 30.15 5.64
        % 24000.00  28.71 10.61 29.42 5.50
        % 25000.00  28.65 10.60 28.70 5.36
        % 26000.00  28.60 10.59 27.99 5.22
        % 27000.00  28.54 10.57 27.33 5.09
        % 28000.00  28.49 10.56 26.71 4.96
        % 29000.00  28.43 10.54 26.12 4.84
        % 30000.00  28.39 10.53 25.54 4.73
        % 31000.00  28.35 10.52 25.02 4.62
        32000.00  28.33 10.51 24.52 4.52
        % 33000.00  28.30 10.49 24.01 4.41
        % 34000.00  28.28 10.48 23.49 4.32
        % 35000.00  28.25 10.47 23.02 4.22
        % 36000.00  28.23 10.47 22.58 4.14
        % 37000.00  28.21 10.46 22.19 4.05
        % 38000.00  28.19 10.45 21.79 3.97
        % 39000.00  28.17 10.44 21.40 3.89
        % 40000.00  28.14 10.43 21.01 3.81
        % 41000.00  28.10 10.42 20.65 3.73
        % 42000.00  28.06 10.40 20.29 3.66
        % 43000.00  28.04 10.39 19.95 3.59
        % 44000.00  28.00 10.38 19.61 3.52
        % 45000.00  27.96 10.37 19.28 3.46
        % 46000.00  27.93 10.36 18.98 3.40
        % 47000.00  27.90 10.35 18.68 3.34
        % 48000.00  27.87 10.34 18.42 3.28
        % 49000.00  27.84 10.33 18.15 3.23
        % 50000.00  27.82 10.32 17.86 3.17
        % 51000.00  27.79 10.31 17.59 3.12
        % 52000.00  27.76 10.30 17.33 3.07
        % 53000.00  27.73 10.29 17.07 3.02
        % 54000.00  27.70 10.28 16.82 2.97
        % 55000.00  27.66 10.27 16.58 2.92
        % 56000.00  27.62 10.26 16.35 2.88
        % 57000.00  27.58 10.25 16.12 2.83
        % 58000.00  27.55 10.24 15.90 2.79
        % 59000.00  27.51 10.23 15.67 2.75
        % 60000.00  27.48 10.22 15.46 2.71
        % 61000.00  27.43 10.21 15.26 2.67
        % 62000.00  27.39 10.20 15.06 2.63
        % 63000.00  27.36 10.19 14.87 2.59
        64000.00  27.32 10.18 14.67 2.56
        % 65000.00  27.29 10.17 14.47 2.52
        % 66000.00  27.25 10.16 14.29 2.49
        % 67000.00  27.22 10.15 14.12 2.45
        % 68000.00  27.19 10.14 13.94 2.42
        % 69000.00  27.16 10.13 13.76 2.39
        70000.00  27.12 10.12 13.60 2.36
    }\ltqTable
    
    \begin{tikzpicture}
        \begin{axis}[
            height=40mm,
            width=1.0\linewidth,
            xmode=log,
            % xmin=1,
            % xmax=16,
            % ymin=0,
            % ymax=150,
            xlabel=Number of Queries $n$,
            xlabel near ticks,
            % ylabel=RMS Error,
            ymode=log,
            ylabel=Latency (ms/op),
            ylabel near ticks,
            ylabel style={align=center},
            % xtick={1, 4, 8, ..., 16},
            % xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
            % ytick={0, 30, 60, 90, 120, 150},
            % yticklabels={0\%, 30\%, 60\%, 90\%, 120\%, 150\%},
            % xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
            % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
            % extra y ticks={10, 20, 30, 40},
            % extra y tick style={yticklabels={}},
            % ylabel shift=-2pt,
            % xlabel shift=-2pt,
            legend style={
                % at={(0.5,1.55)},anchor=south,column sep=2pt,
                at={(0.99,0.97)},anchor=north east,column sep=2pt,
                % at={(0.42,-0.45)},anchor=north,column sep=2pt,
                % at={(1.02,1.0)},anchor=north west,column sep=2pt,
                draw=black,fill=white,line width=.5pt,
                font=\scriptsize,
                /tikz/every even column/.append style={column sep=5pt}
            },
            legend columns=2,
            colormap name=bright,
            every axis/.append style={font=\small},
            xmajorgrids,
            % xminorgrids,
            ymajorgrids,
            % yminorgrids,
            % minor grid style=lightgray,
            % nodes near coords,
            % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
        ]
        
        \addplot+[mark=x]
        table[x=dataset,y=psql] {\ltqTable};
        \addlegendentry{PostgreSQL}
        
        \addplot+[mark=o]
        table[x=dataset,y=rocksdb] {\ltqTable};
        \addlegendentry{RocksDB}
        
        \addplot+[mark=square]
        table[x=dataset,y=rmi] {\ltqTable};
        \addlegendentry{RMI}
        
        \addplot+[mark=diamond]
        table[x=dataset,y=pwl] {\ltqTable};
        \addlegendentry{\system}
        
        \end{axis}
    \end{tikzpicture}
        
    \vspace{-4mm}
    \caption{Average latency over first $n$ queries of different systems on \texttt{wiki} dataset. The plot shows $n \in \{1, 2, 4, \dots, 512, 1k, 2k, 4k, \dots, 64k, 70k \}$. Both axes are in the logarithmic scale.}
    \label{fig:latency_trend}
    \vspace{-5mm}
\end{figure}


==> figures/examples/stacked_barplot.tex <==
\begin{figure}[t]

\pgfplotstableread{
method low high
lucene 859.6774193548387 211.93548387096777
elasticsearch 909.0 572.5
sqlite 629.032258064516 165.1612903225806
hashtable 370.0 817.0967741935484
iou0 220.33333333333331 116.66666666666666
}\dataTransferTable

\centering
\begin{tikzpicture}
    \begin{axis}[
        xbar stacked,
        scale only axis,
        bar width=1.8mm,
        width=0.75\linewidth,
        height=0.25\linewidth,
        xmin=0,
        xmax=2000,
        xtick={0, 500, ..., 2000},
        minor tick num=1,
        xmajorgrids,
        xminorgrids,
        y dir=reverse,
        ytick=data,
        xlabel near ticks,
        ylabel near ticks,
        xlabel=Latency (ms),
        xlabel shift=-1mm,
        % ylabel=Download Time (s),
        yticklabels={Lucene,Elasticsearch,SQLite,HashTable,\system},
        every axis/.append style={font=\scriptsize},
        % legend pos=south east,
        legend style={
            font=\scriptsize,
            at={(0.98,0.05)}, anchor=south east,
            % at={(1.05,0.5)}, anchor=west,
            % draw=none,
            draw=black,
            fill=white
        },
        legend cell align={left},
        % legend columns=1
    ]
        \addplot [
            fill=vintageblack!70
        ] table [x=low, meta=method,y expr=\coordindex] {\dataTransferTable};
        \addplot [
            fill=vintageblack!10,
            % point meta=x,
            % nodes near coords,
            % nodes near coords align={anchor=west},
            % every node near coord/.append style={
            %     black,
            %     fill=white,
            %     fill opacity=0.75,
            %     text opacity=1,
            %     outer sep=\pgflinewidth % so the label fill doesn't overlap the plot
            % }
        ] table [x=high, meta=method,y expr=\coordindex] {\dataTransferTable};
        \legend{Wait Time,Download Time}
    \end{axis}
\end{tikzpicture}
\vspace{-2mm}

\caption{Search latency breakdown in terms of network communication on the \texttt{Spark} dataset. The total search latency is equal to the summation of wait time and download time.}
\vspace{-3mm}

\label{fig:data_transfer}
\end{figure}

% \pgfplotstableread{
% x    y    method
% 0.1  0.15 a
% 0.45 0.27 c
% 0.02 0.17 a
% 0.06 0.1  a
% 0.9  0.5  b
% 0.5  0.3  c
% 0.85 0.52 b
% 0.12 0.05 a
% 0.73 0.45 b
% 0.53 0.25 c
% 0.76 0.5  b
% 0.55 0.32 c
% }\datatable

% \begin{figure}[t]

% \begin{tikzpicture}
% \begin{axis}[legend pos=south east]
%     \addplot[
%         scatter,only marks,scatter src=explicit symbolic,
%         scatter/classes={
%             a={mark=square*,blue},
%             b={mark=triangle*,red},
%             c={mark=o,draw=black,fill=black}
%         }
%     ]
%     table[x=x,y=y,meta=method]{\datatable};
%     \legend{Class 1,Class 2,Class 3}
% \end{axis}
% \end{tikzpicture}

% \end{figure}

==> figures/experiments/archive/II_breakdown_by_layer_local.tex <==

\pgfplotsset{
    breakdown/.style={
        width=0.8\linewidth,
        height=30mm,
        ybar stacked,
        scale only axis,
        bar width=1.8mm,
        axis lines=left,
        axis line style={-},
        y axis line style={draw opacity=0},
        x axis line style={draw opacity=1},
        ymajorgrids,
        yminorgrids,
        ymin=0,
        ymax=120,
        ytick={0, 25, 50, 75, 100},
        ytick style={draw=none},
        yticklabels={},
        enlarge x limits=1.1,
        xtick=data,
        xlabel near ticks,
        xticklabel style={rotate=15},
        symbolic x coords={B-tree, AirIndex},
        every axis/.append style={font=\scriptsize},
        legend columns=1,
        legend style={
            font=\scriptsize,
            at={(1.05,0.5)}, anchor=west,
            draw=black,
            fill=white
        },
        legend cell align={left},
        every node near coord/.append style={yshift=0pt}
    },
}

\pgfplotsset{
    breakdownfull/.style={
        breakdown,
        yticklabels={0, 25, 50, 75, 100},
        ylabel near ticks,
        ylabel=Relative Latency to \btree ($\%$),
        ylabel shift=-1mm,
        y axis line style={draw opacity=1}
    },
}

\begin{figure*}[t]
    \centering
    
    \def\numberyshift{10.0}
    \def\subfigurewidth{0.16\linewidth}
    \def\legendwidth{0.2\linewidth}
    
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-tree	38.7104	7.1136	19.5912	32.1772	97.5924	2.0973	2.0972648	{\numberyshift}
AirIndex	37.4114	0.0000	17.7462	30.4561	85.6138	1.8446	1.8446016	{\numberyshift}
        }\Table
        
        \begin{tikzpicture}
            \begin{axis}[breakdownfull
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\Table};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\Table};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\Table};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\Table};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\Table};
            \end{axis}
        \end{tikzpicture}
        \caption{1st}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-tree	11.4436	8.0608	36.5114	41.9196	97.9354	8.4901	0.849007395	{\numberyshift}
AirIndex	9.4884	0.0000	20.1783	42.9850	72.6517	6.3412	0.63411884	{\numberyshift}
        }\Table
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\Table};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\Table};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\Table};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\Table};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\Table};
            \end{axis}
        \end{tikzpicture}
        \caption{10th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-tree	1.7081	1.6439	32.5672	62.5362	98.4553	48.8935	0.4889347795	{\numberyshift}
AirIndex	1.7542	0.0000	22.8268	58.6038	83.1849	41.4568	0.4145683815	{\numberyshift}
        }\Table
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\Table};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\Table};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\Table};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\Table};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\Table};
            \end{axis}
        \end{tikzpicture}
        \caption{100th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-tree	0.2100	0.2078	28.7395	69.6291	98.7863	405.8741	0.4058741094	{\numberyshift}
AirIndex	0.2084	0.0000	11.6444	67.4674	79.3203	326.1493	0.3261493397	{\numberyshift}
        }\Table
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\Table};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\Table};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\Table};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\Table};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\Table};
            \end{axis}
        \end{tikzpicture}
        \caption{1000th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-tree	0.0269	0.0275	7.8920	90.7044	98.6507	3106.4899	0.3106489902	{\numberyshift}
AirIndex	0.0267	0.0000	1.5748	87.1637	88.7651	2797.7870	0.279778696	{\numberyshift}
        }\Table
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\Table};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\Table};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\Table};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\Table};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\Table};
            \legend{Root Layer, Layer 2, Layer 1, Data Layer}
            \end{axis}
        \end{tikzpicture}
        \caption{10000th}
    \end{subfigure}
\vspace{-3mm}
\caption{Latency breakdown on SSD of \btree and \system by time spent reading different layers. We vary the warmness by the number of queries from left to right. The numbers above the bars are query speed or per-query latency in ms/op.}
\label{fig:II_breakdown_by_layer_local}
\end{figure*}



\pgfplotsset{
    breakdown/.style={
        width=0.8\linewidth,
        height=30mm,
        ybar stacked,
        scale only axis,
        bar width=1.8mm,
        axis lines=left,
        axis line style={-},
        y axis line style={draw opacity=0},
        x axis line style={draw opacity=1},
        ymajorgrids,
        yminorgrids,
        ymin=0,
        ymax=120,
        ytick={0, 25, 50, 75, 100},
        ytick style={draw=none},
        yticklabels={},
        enlarge x limits=1.1,
        xtick=data,
        xlabel near ticks,
        xticklabel style={rotate=15},
        symbolic x coords={B-Tree, AirIndex},
        every axis/.append style={font=\scriptsize},
        legend columns=1,
        legend style={
            font=\scriptsize,
            at={(1.05,0.5)}, anchor=west,
            draw=black,
            fill=white
        },
        legend cell align={left},
        every node near coord/.append style={yshift=0pt},
    },
}

\pgfplotsset{
    breakdownfull/.style={
        breakdown,
        yticklabels={0, 25, 50, 75, 100},
        ylabel near ticks,
        ylabel=Relative Latency to \btree ($\%$),
        ylabel shift=-1mm,
        y axis line style={draw opacity=1}
    },
}

\begin{figure*}[t]
    \centering
    
    \def\numberyshift{10.0}
    \def\subfigurewidth{0.16\linewidth}
    \def\legendwidth{0.2\linewidth}
    
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	24.0180	11.8578	29.3047	34.7809	99.9614	177.1482	177.1 {\numberyshift}
AirIndex	19.4905	0.0000	0.0000	27.3365	46.8271	83.0275	83.0 {\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdownfull
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit,
                ] table [x=method, y=yshift, meta=speed] {\NFS};
                
            \end{axis}
        \end{tikzpicture}
        \caption{1st}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	4.5874	6.9453	31.7869	56.6150	99.9346	818.4797	81.84797339	{\numberyshift}
AirIndex	4.0446	0.0000	0.0000	30.7788	34.8233	285.5671	28.5567098	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \end{axis}
        \end{tikzpicture}
        \caption{10th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
        B-Tree	0.5235	0.9626	24.8073	73.6635	99.9569	6420.2773	64.20277329	{\numberyshift}
AirIndex	0.5396	0.0000	0.0000	16.6856	17.2252	1109.1088	11.0910879	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \end{axis}
        \end{tikzpicture}
        \caption{100th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	0.0644	0.1137	23.9182	75.8720	99.9683	61812.0694	61.81206939	{\numberyshift}
AirIndex	0.0526	0.0000	0.0000	16.7226	16.7752	10395.0381	10.39503806	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \end{axis}
        \end{tikzpicture}
        \caption{1000th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	0.0113	0.0154	6.7720	93.1616	99.9602	451035.5964	45.10355964	{\numberyshift}
AirIndex	0.0088	0.0000	0.0000	23.0508	23.0596	104270.7217	10.42707217	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \legend{Root Layer, Layer 2, Layer 1, Data Layer}
            \end{axis}
        \end{tikzpicture}
        \caption{10000th}
    \end{subfigure}
\caption{Latency breakdown on NFS of \btree and \system by time spent reading different layers. We vary the warmness by the number of queries from left to right. The numbers above the bars are query speed or per-query latency in ms/op.}
\label{fig:II_breakdown_by_layer_nfs}
\end{figure*}



==> figures/experiments/archive/II_breakdown_by_layer_nfs.tex <==

\pgfplotsset{
    breakdown/.style={
        width=0.8\linewidth,
        height=30mm,
        ybar stacked,
        scale only axis,
        bar width=1.8mm,
        axis lines=left,
        axis line style={-},
        y axis line style={draw opacity=0},
        x axis line style={draw opacity=1},
        ymajorgrids,
        yminorgrids,
        ymin=0,
        ymax=120,
        ytick={0, 25, 50, 75, 100},
        ytick style={draw=none},
        yticklabels={},
        enlarge x limits=1.1,
        xtick=data,
        xlabel near ticks,
        xticklabel style={rotate=15},
        symbolic x coords={B-Tree, AirIndex},
        every axis/.append style={font=\scriptsize},
        legend columns=1,
        legend style={
            font=\scriptsize,
            at={(1.05,0.5)}, anchor=west,
            draw=black,
            fill=white
        },
        legend cell align={left},
        every node near coord/.append style={yshift=0pt},
    },
}

\pgfplotsset{
    breakdownfull/.style={
        breakdown,
        yticklabels={0, 25, 50, 75, 100},
        ylabel near ticks,
        ylabel=Relative Latency to \btree ($\%$),
        ylabel shift=-1mm,
        y axis line style={draw opacity=1}
    },
}

\begin{figure*}[t]
    \centering
    
    \def\numberyshift{10.0}
    \def\subfigurewidth{0.16\linewidth}
    \def\legendwidth{0.2\linewidth}
    
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	24.0180	11.8578	29.3047	34.7809	99.9614	177.1482	177.1 {\numberyshift}
AirIndex	19.4905	0.0000	0.0000	27.3365	46.8271	83.0275	83.0 {\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdownfull
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit,
                ] table [x=method, y=yshift, meta=speed] {\NFS};
                
            \end{axis}
        \end{tikzpicture}
        \caption{1st}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	4.5874	6.9453	31.7869	56.6150	99.9346	818.4797	81.84797339	{\numberyshift}
AirIndex	4.0446	0.0000	0.0000	30.7788	34.8233	285.5671	28.5567098	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \end{axis}
        \end{tikzpicture}
        \caption{10th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
        B-Tree	0.5235	0.9626	24.8073	73.6635	99.9569	6420.2773	64.20277329	{\numberyshift}
AirIndex	0.5396	0.0000	0.0000	16.6856	17.2252	1109.1088	11.0910879	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \end{axis}
        \end{tikzpicture}
        \caption{100th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	0.0644	0.1137	23.9182	75.8720	99.9683	61812.0694	61.81206939	{\numberyshift}
AirIndex	0.0526	0.0000	0.0000	16.7226	16.7752	10395.0381	10.39503806	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \end{axis}
        \end{tikzpicture}
        \caption{1000th}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{\subfigurewidth}
        \centering
        \pgfplotstableread{
        method	root	layer_2	layer_1	data	CHECKSUM	total	speed	yshift
B-Tree	0.0113	0.0154	6.7720	93.1616	99.9602	451035.5964	45.10355964	{\numberyshift}
AirIndex	0.0088	0.0000	0.0000	23.0508	23.0596	104270.7217	10.42707217	{\numberyshift}
        }\NFS
        
        \begin{tikzpicture}
            \begin{axis}[breakdown
            ]
                \addplot[
                    fill={rootcolor},
                    text opacity=1] table [x=method, y=root] {\NFS};
                \addplot[
                    fill={layeronecolor},
                    text opacity=1] table [x=method, y=layer_2] {\NFS};
                \addplot[
                    fill={layertwocolor},
                    text opacity=1] table [x=method, y=layer_1] {\NFS};
                \addplot[
                    fill={datalayercolor},
                    text opacity=1] table [x=method, y=data] {\NFS};
                \addplot [
                    opacity=0.0,
                    text opacity=1.0,
                    nodes near coords,
                    point meta=explicit
                ] table [x=method, y=yshift, meta=speed] {\NFS};
            \legend{Root Layer, Layer 2, Layer 1, Data Layer}
            \end{axis}
        \end{tikzpicture}
        \caption{10000th}
    \end{subfigure}
\caption{Latency breakdown on NFS of \btree and \system by time spent reading different layers. We vary the warmness by the number of queries from left to right. The numbers above the bars are query speed or per-query latency in ms/op.}
\label{fig:II_breakdown_by_layer_nfs}
\end{figure*}



==> figures/intro/quadrant.tex <==
\begin{figure}[t]

\hspace*{-4mm}
\begin{tikzpicture}

\tikzset{
mynode/.style={
    font=\scriptsize,
    align=center,
    text width=0.32\linewidth
},
}

\begin{axis}[
    width=75mm,
    height=40mm,
    xmin=0,
    xmax=2,
    ymin=0,
    ymax=2,
    xtick={1,2},
    ytick={1,2},
    xticklabels={Pretuned to Storage, Adaptive to Storage},
    yticklabels={Distribution\\Agnostic, Distribution\\Aware},
    yticklabel style={align=center,yshift=-7mm,xshift=2mm,rotate=60},
    xticklabel style={align=center,xshift=-15mm},
    xlabel=Storage,
    ylabel=Data,
    tick label style={font=\footnotesize\sf},
    label style={font=\footnotesize\bf},
    grid=both,
    minor grid style={solid,gray},
]

\node[mynode] at (axis cs: 0.5, 1.5) {
    RMI~\cite{kipf2018learned}, 
    PGM-Index~\cite{DBLP:journals/pvldb/FerraginaV20PGMIndex}, 
    RadixSpline~\cite{DBLP:conf/sigmod/KipfMRSKK020RadixSpline}, 
    interpolation searches~\cite{DBLP:conf/damon/Graefe2006InterpolationSearch},
    ALEX~\cite{DingMYWDLZCGKLK2020ALEX}
    };

\node[mynode] at (axis cs: 0.5, 0.5) { B-tree~\cite{Bayer1972}, pB${}^{+}$-Tree~\cite{Chen2001}, fpB${}^{+}$-Tree~\cite{Chen2002}, PA-Tree~\cite{Wang2020}, CG-index~\cite{Wu2010}, SNB-index~\cite{Zhou2014}, EDB~\cite{Bin2014}};

\node[mynode] at (axis cs: 1.5, 0.5) {Cache-oblivious B-Tree~\cite{bender2000CacheObliviousBtree}, COLA~\cite{DBLP:conf/spaa/BenderFFFKN2007COLA}, xDict~\cite{DBLP:conf/soda/BrodalDFILM2010xDict}};

\node[mynode] at (axis cs: 1.5, 1.5) {\textbf{Ours (\system)}};

\end{axis}

\end{tikzpicture}

\vspace{-2mm}
\caption{Unlike existing methods, \system adapts to both data distribution and storage performance.}
\label{fig:intro:quadrant}
\vspace{-5mm}
\end{figure}


==> figures/methodology/e2e_bnb.tex <==
\begin{figure*}[t]
  \centering
  \resizebox{\linewidth}{!}{%
  \input{figures/methodology/e2e_bnb_tikz}
  }
  
  \vspace{-2mm}
  \caption{\system automatic tuning algorithm, starting from the bottom (data layer) to the top. The label ``root'' indicates that the candidate should be the root layer with no further index layer, signifying the base case of the recursion. In this illustration, the algorithm selects $k = 3$ top candidates to branch out and finds candidates with $L = 1$ and $L = 2$ layers.}
  \vspace{-3mm}
  \label{fig:branch_and_bound}
\end{figure*}

==> figures/storage_profile.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
      width=0.8\linewidth,
      axis lines=middle,
      grid,
      ymin=0,
      ymax=11,
      ytick={0,...,10},
      xmin=6,
      xmax=23,
      xtick={7,...,22},
    %   xticklabel={\pgfmathprintnumber{\tick}:00},
    %   xticklabel style={rotate=45,anchor=north east}
    ]
    
        \addplot[draw=none] coordinates {(1,1)};
    \end{axis}
    \end{tikzpicture}
    
    \caption{Latency and bandwidth profiles across many storage medias \tofix{Find data and plot log-scale with labels here}}
    \label{fig:dummy_line}
    \vspace{-3mm}
\end{figure}

==> sections/2_background.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Motivation}

% why this is the right time to tune index to specfic storage?

% diversity in storage, cloud environment is even more diverse

% elastic computing

% why existing is suboptimal (example: B-tree) --> depends on storage (require DBA) --> may not update along with storage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivation (remove if not enough time)}

\input{figures/background/motivation}

\subsection{Machine Learning for Indexes}

\todo{Depending on data distribution, there are models/regressors that fit better with;
    explain the difference between B-tree and learned indexes;
        core difference: learned indexes use ``models''.}



\subsection{Need for Also Fitting to Storage}

\todo{Need to answer why these existing approaches are insufficient}

\todo{We consider ``time''. we minimize time to retrieve model + prediction error + time to fetch data in the next layer.}


Tuned B-trees; Select good ones; Learned indexes

Learning objective of the existing work is to minimize the error between data and models.
RMI minimizes XX (e.g., the error between data distribution and piecewise linear functions). 
Method2 minimizes YY;
Method3 minimizes ZZ;
and so on


Why not enough? Have some deeper analysis with a concrete example.
1. RMI may be too shallow for a certain situation . 
    % Depending on bandwidth, for example, the optimal height varies. Why?
    % Larger bandwidth -> Smaller nodes? -> 
    a. Depending on latency, optimal heights differ. <- explain this with concrete examples.
    b. (bandwidth is smaller): bandwidth has similar effect as latency in an opposite direction; that is, as bandwidth increases, we prefer larger models (thus, shallower indexes) <- no need to give concrete examples.
2. error correction



\tofix{Section introduction}

\subsection{Storage and Data Systems}

\tofix{motivation? why do we want to fit against storage?}

\tofix{heterogeneous environment -> manual tuning not work}

\tofix{complexity in understanding storage -> generic empirical profiling is needed}

\tofix{Can we consider variance? Why avg works? easily extended to output variance}



% \subsection{Index (Will be removed)}

% Index is a data structure that takes a key $x$ and locates its relevant position(s) $y(x)$ in a storage. Typically, a key is a completely comparable object such as a number or a string, while a position is an address in the underlying storage for example byte range, page number, or block identifier. Classically, indexes come in many forms. \supawit{<Tree>. <Interpolating tree>. <Skip list>. <Succinct data structure>}

% In recent years, learned indexes have emerged to outperform traditional indexes by capturing patterns in key-position distributions. Two prominent features in learned indexes are 1) generalized model as a function mapping a key to its potential position(s) $\hat{y}(x)$, and 2) error correction (a.k.a. last mile search) to find the true position by exploiting storage properties such as key ordering. \supawit{<RMI> <ALEX> <AIDEL> <FITing-Tree> <PGM-Index>} \supawit{Bourbon, BigTable}


\tofix{Why index on storage?}

\tofix{Limitation of existing learned indexes on storage?}

\tofix{Other possible (worse) approaches: tune b-tree, virtual memory (mmap), lmdb is using mmap}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Reconciliation of Indexes}


==> sections/old_methodology.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{System Overview}
\label{sec:overview}

We describe \system's core components (\cref{sec:overview:archi})
% the current scope of this work (\cref{sec:overview:scope}),
and a storage profile 
    representing I/O performance (\cref{sec:storage_model}).

% system operations

% \tofix{point lookup; why OK?}

% \tofix{why read-only OK? scope: read-only}

% \tofix{deployment under various cloud/storage interfaces}

% storage related

% \tofix{storage dominates latency}

% \tofix{storage model (abstraction)}

% \tofix{What is storage profile? function: sequential bytes -> time, Why generic function (not simple ones)}

% \tofix{What if storage profile significantly drifts over time?}

% \tofix{Variance in storage performance}


\subsection{Architecture}
\label{sec:overview:archi}

\input{figures/methodology/architecture}

\system is an index library for sorted key-value data stored on \fixed{a} Storage Layer (e.g., SSD, NFS).
\system can work with various storage devices/services by extending its storage interface.
    % as described shortly.
\system stores indexes together with the data on Storage Layer
    while part of them may be cached.
Internally,
\system consists of three components---Lookup, Builder, and Storage Layer Interface---as
    depicted in \cref{fig:architecture}.
First, Storage Layer Interface provides the consistent abstraction over different storage interfaces/devices
    (e.g., virtual file systems (VFS), over SSD or object storage, cloud storage services)
    such as creating files
        and reading/writing serialized objects.
Based on this consistent interface, we can profile
    the time needed to read $\Delta$ bytes (\cref{sec:storage_model}).
%
Second, Lookup provides a querying interface.
    Given a key,
        the module traverses an index
    as it fetches necessary data (e.g., ranges within index layers) if not cached,
        caches the fetched data if space is available (\cref{sec:data_layout}),
    and makes inferences on what data it needs to fetch next (\cref{sec:querying}),
until it finds the value associated with the key (or if finds there are no such keys indexed).
%
Finally, Builder finds optimal index designs and
    builds/stores actual indexes on storage (\cref{sec:system-building-overall,sec:system-building-node-estimation,sec:system-building-selection}).
How Builder finds high-quality index designs efficiently
    is the key contribution of this work.

% \system disaggregates compute and storage. The storage keeps all states including data collections and serialized index structures. On a compute node, a \system client executes the lookup procedure by accessing the storage when necessary. The client is expected to be short-lived and/or has a limited memory relatively to the amount of data. In these large-scale resource-limiting scenarios, caching would be ineffective, and so, \system is optimized for cache-free cases where no information is stored locally apart from the storage. \system is suitable for a serverless deployment. 


\ignore{
\subsection{Current Scope}
\label{sec:overview:scope}

% What kinds of operations we improve: key(?) lookup
\paragraph{Point lookup \& Range Query}

Given a search key, \system retrieves an associated value (if the key exists)
    by identifying a byte offset range within indexed data
        containing the search key.
Like many others~\cite{kipf2018learned,DBLP:journals/pvldb/FerraginaV20PGMIndex, DBLP:conf/sigmod/KipfMRSKK020RadixSpline,DingMYWDLZCGKLK2020ALEX}, \system indexes sorted data;
    thus, point lookup can easily be extended
        to support range queries.
% retrieve a key's position in a data collection persisted on a storage. To accelerate the lookup beyond traditional approaches, it utilizes the learned index---a concept that has found successes on internal memory---and integrates it onto the external storage. Although learned index opens wider possibilities of configurations, \system can efficiently and accurately find the right setting for the storage with a unique performance.


\paragraph{Indexes for Key-Value Stores}

While \system's indexes are not updatable---disallowing 
    in-place updates---\system
        can be used for general, updatable data systems 
    such as LSM tree-based KV stores~\cite{rocksdb,Raju2017},
    an important class of data systems
        widely used in practice.
To offer fast random accesses,
those systems build indexes as part of their merge operations,
        which produce larger key-value segments
    by sort-merging existing ones.
The data in a segment does not update
    until they are merged into a longer segment,
        which makes \system suitable for those systems.
}
% Before serving any query on a data collection, \system examines the storage and data distribution, optimizes its configuration, and writes the index structure to the storage. \system, therefore, targets immutable data collections. Even so, it can be augmented to infrequently mutating data by periodically rebuilding and appending data by applying \system on each node in a log-structure merge-tree (LSM-Tree)~\cite{DBLP:journals/acta/ONeilCGO96LSMTree} during compaction.


% \paragraph{Variance in Storage Model}
% \todo{Describe something here}


\input{figures/methodology/notation_table}


\subsection{Storage Model}
\label{sec:storage_model}

% \todo{Describe interface also. Is the storage supposed to be a file system-like interface?}

\system operates on a \emph{storage performance profile} $T(\Delta)$, which represents 
    the time taken for a storage device/layer to read consecutive data of size $\Delta$ bytes. 
Storage model captures \textit{locality} where accessing contiguous data is faster than accessing data from different  locations. 
% For a popular example, spinning disk HDD accesses data by aligning its circular storage medium with a stationary needle reader. By physically spinning the medium a position away, it can read data in the next block. However, to reach for data far away, the HDD has to rotate more, incurring more seek time.
In the simplest case, $T(\Delta)$ can be an affine function $T_{\text{aff}}(\Delta) = \ell + \Delta / B$ whose two parameters are latency $\ell$ and bandwidth $B$.
While we employ this storage model to analyze \system's behavior in terms of 
    two simple parameters---$\ell$ and $B$---our optimization process
        can work with any monotonically increasing $T(\Delta)$.

% To fit this affine storage profile, one could measure the latency $\ell$ using a small $\Delta$ and infer the bandwidth through another measurement of a bigger $\Delta$. 
% \cite{DBLP:journals/csur/Vitter2001ExternalMemoryModel} delves deeper into different models such as disk access model, parallel external memory model, and parallel disk model. 
% From this point on, we may refer to external memory and storage interchangeably.

Currently, we consider a deterministic and time-independent $T(\Delta)$,
    summarizing over
        other variables---such as address alignment, prefetching states,
            low-level optimizations, and storage age---which
    % requiring summarization over other neglected variables such as address alignment, prefetching states, low-level optimizations, and storage age 
    are difficult to infer/generalize for index systems.
To obtain accurate $T(\Delta)$,
% For example of a summarization, 
    one could quantize $\Delta$ domain, measure the latency, and summarize the measurements 
        with averages or medians. 
\fixed{
    Despite being out of scope,
        we can extend $T(\Delta)$ from a deterministic function to a distribution function conditioned on the read size $\Delta$.
    Apart from becoming more realistic, this storage model would enrich \system to tune on more complex goals such as fastest tail latency (e.g., lowest p99) or highest reliability (e.g., lowest latency variance).
}

% Despite being out of scope, non-deterministic storage models may apply to parts of our methodology with appropriate modifications to incorporate effects of randomness like optimizing for low-variance indexes. 
% All in all, we believe that $T(\Delta)$ is the right level of abstraction to reason about index structures.

% \input{figures/storage_profile}

% \begin{itemize}
%     \item{Hard Disk Drives}: Describe seek time, page read, behavior
%     \item{Solid-state Drives}: NAND, block-based, microsecond latency
%     \item{Network File Systems}: distributed file system, \href{https://www.semanticscholar.org/paper/The-Sun-Network-Filesystem\%3A-Design\%2C-Implementation-Sandberg/1b07afcb4e1b4d94dcb537589db1a2653f14e887}{SUN (1984)}
%     \item{Cloud Storage}: Blob storage, protocol and latencies. Examples in AWS, GCP, Azure.
%     \item{(Remote) Direct Memory Access?}
% \end{itemize}

% Latency and bandwidth both have physical and technological limitations. For one, the speed of light dictates the minimum latency accordingly to distance between compute and storage. Meanwhile, existing materials restricts the largest bandwidth the compute-storage connection can possess. \supawit{explain more on tech limits}. Therefore, external memory model and algorithms will be relevant for the foreseeable future, especially for large data systems. \supawit{generalize read requests} \supawit{$T$ as a summarization of random variable} \supawit{in-memory efforts: XIndex, but we are different}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\ourmodel: Unified Index Model}
\label{sec:system-overall}

In this section,
    we mathematically model hierarchical indexes
        by representing them with design parameters $\bfTheta$,
    which are also used to express their lookup latencies.
These mathematical models
    are the foundations of our optimization process described in \cref{sec:system-building}.

% This section lays out \system's class of indexes that supports a well-structured parameter space. Within this parameter space, Section \cref{sec:system-building} explains how \system searches for the optimal index parameters to build a fast index tuned to the storage by finding $\bfTheta$ that minimizes the storage model cost. Lastly, Section \cref{sec:system-analysis} extensively justifies claims throughout earlier parts while \cref{sec:system-implement} lists down details to implement \system.


\subsection{Target Class of Indexes}
\label{sec:system-overall-class-of-index}

% Previous:
% 1. What we do
% 2. Claim what we do incorporate existing indexes

% Previous Previous:
% 1. We generalize all indexes
% 2. We pick a specific choice

% Proposal:
% 1. Why we want to generalize existing indexes: explain existing indexes are good if choices are well made.
% 2. In order to achieve the goal, we develop/propose/abstract in a certain way, which is the following:

% Good index structures fit well to both data and storage.
% Luckily, many existing indexes already have appropriate templates that capture performant indexes structures; however, their parameterizations often focus on either data or storage, complicating the reasoning when considering both.
% % For example, they can compress the data at the right angle and resolution with respect to index search. They can also express a prior on key-position pattern as a concise model.
% % Many indexes optimized for different storages.
% We collect many data-driven indexes and simplify them from the perspective of our storage model. Doing so, we can formulate the index structure space as well as the well-behaved objective function to be optimized by \system.

\system aims to
    build high-speed \emph{hierarchical indexes},
        a general form of indexes that can encompass many existing indexes,
    while maximizing the opportunity to vary many aspects of those indexes.
A hierarchical index consists of $L$ \textit{index layers}---$I_1, I_2, \ldots I_L$---over 
    a data layer ($D$);
% For a $L$-layer structure, 
    $I_L$ refers to the root, $I_1$ refers to the bottom-most one (closest to the data layer),
        and $I_0$ refers to the data layer $D$.
For each lookup operation,
    a lookup process traverses all the layers starting from the root down to the data layer,
        fetching some or all of their data (unless cached)
    where ranges of data to fetch for $I_l$ are determined by
        its parent layer (= $I_{l+1}$).
For the root ($I_L$), the entire layer needs to be fetched (thus, it is typically cached).

% In the same way a key has a relevant position in the data layer, the key also has a relevant position in each index layer that stores the relevant \textit{node}. A relevant node can map the key to its possible range of positions below, creating a chain of search relationships downward across layers.
% A layer is responsible for searching in the layer below, and so on. The bottom-most layer is responsible for searching relevant data in the data collection. From the perspective of storage usage, each index layer makes exactly one I/O access per search.


\input{figures/methodology/structure}

% Amidst numerous design choices, many of traditional and learned indexes are hierarchical indexes. 
% B-trees are one example.
% Many learned indexes fit into hierarchical index. \supawit{For example, RMI range index~\cite{kipf2018learned}}

% Summarize them in complexity table and in 2D plot (with Pareto front depending on hyperparameters). Explain how to external memory model dictates which solution is the best (hint: dot product). Teaser our Pareto front here if fully covers all indexes, maybe?

% \paragraph{On Error Correction}
% Under hierarchical index point of view, error correction is considered an implicit index layer(s). \supawit{equivalences on binary search and exponential search}

% A particular choice of error correction algorithm implies the predicted position distribution. \supawit{binary search --> bounded uniform distribution, exponential search --> exponential distribution} \supawit{both are considered entropy minimizing methods that check the point $y$ where $\Pr[Y \leq y] = \Pr[Y \geq y]$}


\subsection{Index Layers and Nodes}
\label{sec:data_layout}

The overall structure of
an \system comprises \textit{metadata} and \textit{index layers};
    each layer, in turn, comprises \textit{nodes}. 
% \system preserves the original data collection, 
%     avoiding data rewrite and a bulk of redundant storage cost.

\paragraph{Metadata} 
% To persist and later reconstruct its internal data structures, 
\system's metadata 
encodes index structure, node types, and resource identifiers (e.g., file paths, object names). To avoid an extra round-trip, \system physically stores the root layer and metadata in the same location.
% where \system can read together. 
For example, the root layer and metadata are in the same file on a local SSD
% file-system storage 
    whereas they are in the same blob on an object store. 
Metadata is negligibly small in size relative to the root layer for our optimization.
% and is negligible to the optimization objective. 
% \cref{sec:system-implement-metadata} describes the metadata format in more details.

\paragraph{Index Layer}
An index layer represents a collection of \textit{nodes}, which partitions the key space in data; 
that is, each node is in charge of an exclusive key range
    while the union of those key ranges cover all the keys in the data.
% Not only are the key ranges exclusive, but together they form a complete key space covering all the keys in the data. 
Each layer consists of the same type of nodes (node types are described shortly)
    to simplify layer constructions
        and to prevent the large cost of including extra information within each node,
    which also enhances lookup speed.
% \system uses exactly one node type in each layer. 
    % Apart from simplifying layer constructions, 
% this decision reduces the space per node leading to a saving in storage cost and speedup during search. Moreover, it establishes a naturally aligned physical format, convenient for arbitrary range reads.
In its serialized form, a layer is a series of nodes, arranged back to back;
    each node encodes a learned branching function and the lower end of the key space covered by the function.
    % a a starting key and the node's raw bytes.
% Each node covers a part of the key space, starting from the key encoded in the 
A node's upper end of the key space can be obtained by looking at the next node in the same layer,
    which is similar to B-tree's separator keys.
% Two consecutive separator keys constitute the key range of the node in between, similarly to B-tree's separator keys. 
% For example, 
Based on this structure, we can decode/deserialize the nodes contained within an arbitrary byte range, as follows.
Suppose a key is an $8$-byte integer and the layer contains $100$ nodes with each node taking $40$ bytes.
% of type \texttt{band} whose raw size is $40$ bytes. 
Among the total $100 \times (8 + 40) = 4.8$ KB for the layer,
% The total size of the serialized layer is then $100 \times (8 + 40) = 4.8$ KB. 
a range read over $[48, 480)$ byte range (zero-based), for example, will fetch 2nd to 10th nodes along with their key ranges.
% \supawit{do we need page alignment hypothetical?}
% Each layer, after serialization, is stored in a unique location.
Different layers are stored using separate objects---an $L$-layer index is stored in $L$ files on file-system storage
        or in $L$ objects on blob storage---while the root layer additionally contains the metadata.
% After serializing the layers, \system stores each layer in a unique location. 
% That is, for an $L$-layer index, \system creates $L$ files on a file-system storage. 
% The only exception is the file containing the root layer which additionally contains the metadata.


% node as a blackbox, properties (explain why completely encapsulate)
\paragraph{Node} 

A node is the smallest functional component. 
Given a key $x$ in its corresponding key range, a node predicts a position $\yh: \calX \rightarrow \calY$ in range that encompasses the actual position $y(x)$.
\begin{equation} \label{eq:node-interface}
    \text{Node}\;\yh: \quad \yh(x) = [\yh^{-}(x), \yh^{+}(x)) \supseteq [y^{-}(x), y^{+}(x)) = y(x)
\end{equation}
All nodes in a layer together represents the global function from the key space $\calX$ to position space $\calY$ on the next layer. This decomposability from layer to nodes is a crucial property to enable a partial range read---a core operation in a hierarchical index.

\begin{figure}[t]
  \centering
%   \vspace{2mm}
  % Adjust font size in `pretex=`
  \includesvg[width=0.9\linewidth,pretex=\footnotesize]{figures/methodology/node_types}
%   \includegraphics[width=0.9\linewidth]{figures/methodology/node_types.png}
  \vspace{-2mm}
  \caption{\fixed{Two node types with key-position examples. Left: 5-piece \texttt{step}. Right: \texttt{band} with points and width.}}
%   \vspace{-5mm}
  \label{fig:node_types}
\end{figure}

While our optimization framework can support any such function that implements $\yh$ specified in \cref{eq:node-interface},
    \system currently implements two types of nodes sketched in \cref{fig:node_types}. 
First, a step node (\texttt{step}) is a step function, or a $p$-piece constant function parameterized by partition keys $\bfa = (a_1, \dots, a_p)$ and partition positions $\bfb = (b_1, \dots, b_p)$. In other words, $\yh_{\texttt{step}}(x; \bfa, \bfb) = [b_i, b_{i+1})$ for $x \in [a_i, a_{i+1})$. Second, a linear band node (\texttt{band}) is a thick linear function traveling through two key-position points $(x_1, y_1)$ and $(x_2, y_2)$ with a width $\delta$: $\yh_{\texttt{band}}(x; x_1, y_1, x_2, y_2, \delta) = [m x + c - \delta, m x + c + \delta)$ where $m = (y_2 - y_1) / (x_2 - x_1)$ and $c = y_1 - m x_1$. A step node is $16p$ bytes in size while a linear band node is $40$ bytes.
\fixed{
    For example, consider a dataset with 4 key-position pairs: $D = \{(x, y)\} = \{ (1, [0, 10)), (4, [10, 20)), (5, [20, 25)), (7, [25, 35)) \}$ as in \cref{fig:node_types}. A $\texttt{step}$ node can represent this key-position collection with $p = 5$, $\bfa = (1, 4, 5, 7, \infty)$, and $\bfb = (0, 10, 20, 25, 35)$, guaranteeing the exact prediction $\yh_{\texttt{step}}(x; \bfa, \bfb) = y$ for all $(x, y) \in D$. Note that a $\texttt{step}$ node having fewer pieces can be valid but would have a higher error. Alternatively, a \texttt{band} node can approximately represent $D$ with $(x_1, y_1) = (1, 0), (x_2, y_2) = (4, 10), \delta = 15$. We encourage readers to verify that $\yh_{\texttt{band}}(x; 4, 0, 7, 25, 35) \supseteq y$ for all $(x, y) \in D$.
    % https://www.desmos.com/calculator/ogpq72mvds
}

\fixed{
    Currently, these two node types are sufficient. Together, they efficiently fit sorted key-position collections. \texttt{step} adapts to discontinuities while \texttt{band} regresses well with regularly sized key-value pairs~\cite{pmlr-v119-ferragina2020WhyLearnedIndexWork}. Furthermore, with these types, \ourmodel can already incorporate many existing learned indexes such as PGM-Index~\cite{DBLP:journals/pvldb/FerraginaV20PGMIndex}, ALEX~\cite{DingMYWDLZCGKLK2020ALEX}, RadixSpline~\cite{DBLP:conf/sigmod/KipfMRSKK020RadixSpline}, SIndex~\cite{Wang2020SIndex}, XModel~\cite{Wei2020FastCacheXStoreXModel}.
}

% % \paragraph{Extensibility (\todo{This can be sub of Node})}
% Although \system deploys these two nodes in this work, it can easily 
%     expand supported node types and relax some layer design decisions when appropriate.
% In general, \system requires a layer that 
%     1) decomposes into smaller nodes, 
%     2) is serializable, and 
%     3) predicts completely inclusive position range (i.e., $\yh(x) \supseteq y(x)$).
% Some examples of layer design relaxation include allowing multiple node types within a layer or variable-length raw format. 
% The former requires attaching a type label to each node 
%     while the latter requires an alignment to enable arbitrary range reads.
% This extensibility allows us to
%     easily enhance the expressiveness of indexes
%     without reinventing the optimization framework. \supawit{TODO: Remove this?}
%         % under the same optimization framework.
% % is important to incorporate prior on the target data layout and capture patterns in key-position distribution.

% To operate with an external memory, the node type must be able to serialize a node into raw bytes and deserialize raw bytes to a node.
% \supawit{inclusive from underlying key-position. For a key $x$, the responsible subnode $\yh(x)$ in a particular layer outputs potential positions in a bounded range $\yh(x) = [\yh^{-}(x), \yh^{+}(x)]$ that fully contains the true position $y(x) \in \yh(x)$. As a result, the precision is then $\Delta(x) = \yh^{+}(x) - \yh^{-}(x)$.}
% \supawit{why completely capture? why no error correction and prefer explicit?} \supawit{two nodes fit nicely, these nodes cover extreme cases (best/worst case claim)}

% remind that this list can be expanded to express prior in key-position curve... we pick these because?


% \paragraph{Generalizability}
% \tofix{Our index model can express many things.}

\paragraph{Parameters}
    \system defines $\bfTheta$ as the collection of all parameters sufficient to represent a hierarchical index instance. In particular, $\bfTheta$ specifies the number of layers $L$ followed by $L$ layer-wise parameters $\Theta_i$ which in turn specifies the node type, number of nodes $n_l$, and all node parameters.
\begin{equation} \label{eq:bftheta_parameter}
    \bfTheta = (L, (\Theta_1, \dots, \Theta_L)), 
    \quad 
    \Theta_l = (\texttt{NodeType}, n_l, (\theta_1, \dots, \theta_{n_l}))
\end{equation}    
Node-specific parameters $(\theta_1, \dots, \theta_{n_l})$ for $n_l$ nodes depend on the corresponding $\texttt{NodeType}$. 
For example, if $\texttt{NodeType} = \texttt{step}(p)$, $\theta_i = (\bfa_i, \bfb_i)$ where $|\bfa_i| = |\bfb_i| = p$. If $\texttt{NodeType} = \texttt{band}$, $\theta_i = (x^{(i)}_1, y^{(i)}_1, x^{(i)}_2, y^{(i)}_2, \delta_i)$. We choose to specify a single node type per layer over multiple node types per layer because 
(1) it reduces the serialization overhead per node which reduces read volume and so overall lookup latency, and 
(2) it simplifies the node-building process (\cref{sec:system-building-node-estimation}). Moreover, compared to specifying one global node type across layers, decoupling node types across layers allows \system to fit better to wider families of datasets with negligible storage and latency overhead.


% query process, in algorithm block?
\subsection{Query Process}
\label{sec:querying}

\input{figures/methodology/query_algorithm}


\Cref{algo:query-process} summarizes \system's overall query process, traversing through the index hierarchy of relevant node(s) $\yh_L, \dots, \yh_0$ to retrieve the relevant key-value $(x, v)$. At the start of each iteration, \system is aware of the next position $\yh_l(x)$ to read from. For example, at the beginning of the first iteration ($l = L$), \system aims to read the entire root layer while \system aims to read from the data layer in the last iteration ($l = 0$).

\system iteratively reads potentially relevant keyed raw bytes $\{(x[i], v[i])\}_i$ and finds the relevant raw bytes $v_l$ using local binary search. If the current layer is an index layer $(l \geq 1)$, \system deserializes $v_l$ to reconstruct the next relevant node $\yh_{l-1}$ to predict the next position $\yh_{l-1}(x)$. 
If the current layer is a data layer $(l = 0)$, \system returns the raw bytes with the query key $(x, v_0) = (x, v)$.

% In the implementation, 
% \system reads both the root layer together with the metadata (containing the number of layers) to minimize storage access (\cref{sec:system-implement}). \cref{algo:query-process} omits this detail for brevity.
% to be explained further in .

% Given a query key $x$, 
% % \system parses the dataset's information and 
%     \system accesses the storage to read the root layer together with the metadata,
% which provides the number of layers and the node types in each layer.
% % it reconstructs a lightweight internal data structure to facilitate the search. 
% Then, \system sets the root layer as the current \textit{layer view}. 
% All these processes incur a single storage access.

% \system then sequentially follows the index hierarchy until it reaches the data layer. In each index layer, it finds the relevant node's raw bytes $v_l$ in the current layer view using local binary search, deserializes the raw bytes into an node object $\yh_{l-1}$ (in memory),
%     predicts the next position range $\yh_{l-1}(x)$ using the node, 
%     reads the next layer view in the predicted range from the storage, and 
%     repeats the same process in the layer below. 
% Finally, \system searches for and delivers the relevant key-value in the data layer ($l = 0$). 
% % If the data layer allows, 
% %     \system performs an internal binary search over the layer view. 
% % Otherwise, the data collection user can accept the layer view (or the position range) and proceeds accordingly.


\subsection{Latency Under Storage Model}
\label{sec:objective}

\supawit{TODO: Highlight \cref{algo:query-process} in translation to latency}

Let $\calL(x; \bfTheta, T)$ be the total time it takes to find a value for a key $x$. 
% According to the query process 
As described in \cref{algo:query-process}, 
$\calL$ consists of $L + 1$ terms respectively to the $L + 1$ iterations. Each iteration incurs three kinds of costs:
    storage access $\calL_{SM}$, 
    cache lookup $\calL_{\text{cache}}$,
    % with a cache hit random variable $C$, 
    and 
    internal computation $\calL_{\text{compute}}$.
The former two refers to the storage access (\cref{algo:query-process}, line 2), while
the internal computation includes searching for relevant value, deserializing data, and predicting the next position using the nodes.
Then, $\calL(x; \bfTheta, T)$ can be expressed as:
\begin{align} 
% \begin{alignedat}{-1}
\calL(x; \bfTheta, T) & = 
    \sum_{l=0}^{L} \left(
        (1 - C_l)\, \calL_{SM, l} + C_l\, \calL_{\text{cache}, l} + \calL_{\text{compute}, l} 
    \right) \label{eq:original-cost} \\
    & \leq \sum_{l=0}^{L} \calL_{SM}(x; \Theta_{l+1}, T) + c_{\text{compute}}
\label{eq:emm-totalcost}
% \end{alignedat}
\end{align}
where $C_l$ is a binary random variable that indicates a cache hit ($C_l = 1$) or a miss for the $l$-th layer.
\cref{eq:original-cost} is upper-bounded by \cref{eq:emm-totalcost}---using $c_{\text{compute}}$,
    a constant representing (negligible) compute cost---effectively expressing 
        the end-to-end latency when no data is locally cached, which \system aims to minimize
    by tuning $\bfTheta$,
    to build an index that can offer consistent performance even in the worst case
(\cref{sec:discussion} discusses minor changes needed for
    cache-aware optimization).
$\calL_{SM}(x; \Theta_{l+1}, T)$
    already includes a storage profile $T(\Delta)$;
thus, \cref{eq:emm-totalcost}
    generalizes to different types of storage mediums such as HDD, SSD, NFS, cloud storages, etc.

% In this work, we aim to optimize for the cold-state latency; we consider the maximal cache miss $C = 0$ resulting in an upper bound in \cref{eq:emm-totalcost}, assuming storage access time dominates cache lookup time. Later, our experiment shows that cold-state optimization is relevant up to a wide range of warmness.

% In storage model, the cost to access the external storage $\calL_{SM}(x; \bfTheta_l, T)$ dominates the total computation cost. An external memory (or storage) refers to the slowest storage media in the environment. Some mediums examples includes hard disk drives (HDD), solid-state drives (SSD), remote direct memory access (RDMA), network file systems (NFS), and cloud storages, whose latency is at least in ten microseconds. This is in contrast to internal memory such as CPU caches, RAM, and non-uniform memory access (NUMA) with latency ranging from sub-nanosecond to hundreds of nanoseconds. In a presence of accesses to storage, the cost of internal computations upper bounded by $c_{\text{compute}}$ (e.g., tens of nanoseconds to microseconds for index searching) is negligible. In summary, \system tunes $\bfTheta$ to minimize $\calL_{SM}(x; \bfTheta, T)$.

Next, we extend \cref{eq:emm-totalcost}
    to capture the amount of data we partially read within each layer
    and its impact on the total cost.
The amounts of partial reads
    depend on actual data distributions and the effectiveness of nodes in succinctly capturing those distributions
        into predictors.
We formalize this data- and node-dependent cost
    using a new concept called \emph{precision} $\Delta(x; \Theta_{l+1}) = |\yh_l(x)|$---
    the read size in bytes on a key $x$ for the $l$-th layer. As a special case, $s(\Theta_L) = \Delta(x; \Theta_{L+1}) = |\yh_L(x)| = |\yh_L|$ refers to the size of the $L$-th layer (i.e. the root). We write $\calL_{SM}(x; \Theta_{l+1}, T) = T(\Delta(x; \Theta_{l+1}))$ as the time to read $\Delta(x; \Theta_{l+1})$ bytes, extending \cref{eq:emm-totalcost} into:
% According to the query process, A $L$-layer index accesses the storage exactly $L+1$ times: once to retrieve the root layer ($L$-th layer) and $L$ times to partially read subsequent layers ($L-1$-th, $\dots$, 1st, $0$th layers). Let $\Delta(x; \Theta_l)$ be the \textit{precision} (i.e. read size) in bytes of the $l$-th layer on a key $x$, \system calculates the search cost of a $L$-layer hierarchical index with parameters $\bfTheta = (\Theta_1, \dots, \Theta_L)$ concisely using the storage model cost $\calL_{SM}$ in \cref{eq:emm-hierindex}. 
\begin{equation} \label{eq:emm-hierindex}
    \sum_{l=0}^L \calL_{SM}(x; \Theta_{l+1}, T) = T(s(\Theta_L)) + \sum_{l=1}^L T(\Delta(x; \Theta_l))
\end{equation}
Finally,  
we find the optimal design parameters $\bfTheta^{*}$ 
    that minimizes the expected cost 
    $\calL_{SM}(\calX; \bfTheta^{*}, T) = \E_{x \sim \calX} \calL_{SM}(x; \bfTheta^{*}, T)$:
    % in \cref{eq:emm-obj-airindex} 
\begin{equation} 
\label{eq:emm-obj-airindex}
    \bfTheta^{*} = \argmin_{\bfTheta} \E_{x \sim \calX}\left[ T(s(\Theta_L)) + \sum_{l=1}^L T(\Delta(x; \Theta_l)) \right]
\end{equation}
where $\calX$ is the query key distribution. 
In this work, we set
% In this work, we assume 
$\calX$ to be a uniform distribution over existing keys,
    effectively minimizing the average latency over the entire key set.
% in the data collection $D = \left\{ (x_i, y_i) \right\}_{i=1}^n$. 
% In other words, \system minimizes the average latency over the key set. 
Alternatively, $\calX$ can be set to reflect the target workload if it is known at index build time. 
% We can also write a pessimistic objective function that focuses only on an adversarial key $\argmax_x \Delta(x; \Theta_l)$ across all layers.

% \fixed{
    \input{figures/methodology/opt_summary}
% }
\supawit{TODO: mention optimization summary table (\cref{tab:opt_summary})}

Finding the optimal $\bfTheta$ is a complicated task.
The possibilities of index structure expand a prohibitively large search space to be explored. Not only does \system need to decide the number of layers $L$, but it also needs to determine the node type as well as each node's parameters across all index layers.
Furthermore, these parameters are dependent upon each other, as described in \cref{sec:intro}.
% For example, a change in separator keys on a layer renders the parameters in layers above obsolete.
% A particular pattern in separator keys can favor a particular node type, which is difficult to anticipate until after fitting.
% Adding or removing the number of nodes can also burden or ease the upper layer respectively.


% % problem, cost, search space, hardness
% \subsection{Objective Function}
% \label{sec:system-building-objective}

% \system automatically tunes its index structure onto a data collection with respect to the underlying storage. An index structure is summarized by $\bfTheta = (\Theta_1, \dots, \Theta_L)$ where $\Theta_l$ represents the $l$-th index layer containing separator keys and parameters in all nodes. The structure possibility expand a prohibitively large search space to be explored. Not only does \system need to decide the number of layers $L$, but it also needs to determine per layer the node type as well as each node's parameters.

\fixed{
    \subsection{Hierarchical Index Examples}
    
    As a general class of indexes, hierarchical index examples include traditional indexes like B-tree and learned indexes like \rmi, \pgm, balanced \alex, and \plex. For example, 2-layer balanced B-tree with fanout 3 is a hierarchical index as in \cref{eq:btree-as-hindex} where $\theta_{i,j}$ and $\theta_{k}$ are appropriate step function parameters to encode keys and pointers in the leaf and root nodes respectively.
    \begin{equation} \label{eq:btree-as-hindex}
    \begin{gathered}
        \bfTheta_{\text{B-Tree}} = (2, (\Theta_1, \Theta_2)), \\
        \Theta_1 = (\texttt{step}, 3^2, (\theta_{i,j})_{i,j \in \{1, 2, 3\}}), \\
        \Theta_2 = (\texttt{step}, 3, (\theta_1,\theta_2,\theta_3))
    \end{gathered}
    \end{equation}
    
    \rmi with a cubic root node $ax^3 + bx^2 + cx + d$ and 8 linear intermediate nodes $(\alpha_i x + \beta_i) \pm \varepsilon_i$ is a hierarchical index as in \cref{eq:rmi-as-hindex}. \pgm, balanced \alex, and \plex can be similarly instantiated as hierarchical indexes by extending the node types.
    \begin{equation} \label{eq:rmi-as-hindex}
    \begin{gathered}
        \bfTheta_{\text{\rmi}} = (2, (\Theta_1, \Theta_2)), \\
        \Theta_1 = (\texttt{linear}, 8, ((\alpha_i, \beta_i, \varepsilon_i))_{i \in \{1, \dots, 8\}}), \\
        \Theta_2 = (\texttt{cubic}, 1, ((a, b, c, d)))
    \end{gathered}
    \end{equation}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \section{\oursearch: Optimization with Bounded Visits}
\section{\oursearch: Search with Bounded visits}
\label{sec:system-building}

% \input{figures/methodology/e2e_bnb}

% \begin{figure*}[t]
%   \centering
%   \input{figures/methodology/workflow}
%   \vspace{-2mm}
%   \caption{Overall \system tuning workflow. \supawit{Draw plots} \supawit{Annotate with data layer, $\Theta_1, \Theta_{L=2}$}}
%   \label{fig:workflow}
% \end{figure*}

% \tofix{optimization/build process}

% \tofix{can be random variable}

% \tofix{build complexity analysis}

% \tofix{optimization quality/error}

% \system's design choices set up an orderly configuration space. Especially, its explicit index layer, read-range-addressable layer format, and requirements for types of nodes lay the groundwork to formulate an optimization problem. Although these choices restrict the set of possible index structures, \system still have to determine many more configuration variables, such as number of layers, layer-wise precision, node types, node parameters, and key space partitioning. 
This section describes 
    \system's optimization process (called \oursearch), which
        solves \cref{eq:emm-obj-airindex}.
We first provide a high-level description of the process (\cref{sec:system-building-overall}),
    which is explained further
        by describing node building algorithms (\cref{sec:system-building-node-estimation}),
    quality-guaranteed pruning technique for computational efficiency (\cref{sec:system-building-selection}),
    and parallelization technique (\cref{sec:system-building-parallelism}).
Finally, we present time-complexity analysis (\cref{sec:system-analysis}).

% the core \system's tuning algorithm (\cref{sec:system-building-overall}), explains some steps in details (\cref{sec:system-building-node-estimation} and \cref{sec:system-building-selection}), and points out parallelism opportunities to accelerate the tuning.


% explain the bottom-up approach in top-down fashion: drafts -> select -> write
\subsection{Guided Graph Search}
\label{sec:system-building-overall}

\supawit{TODO: reference \cref{fig:branch_and_bound}} \supawit{TODO: add concrete example on the graph search}

% No way to tell which node builder is the best
% Built index layer may exhibit a different key-position pattern
% The overall building methodology described in 
In \oursearch's search process, 
% resembles SMA*~\cite{russel1992effcient} 
a state represents the current 
    candidate design (indexing $D$)
% key-position collection $D$ 
while the traversal decisions consist of different \emph{node builder} (\cref{sec:system-building-node-estimation}) to build the next layer $\Theta_{\text{next}}$.
Later, the next layer $\Theta_{\text{next}}$ is outlined into the next key-position collection $D_{\text{next}}$ where each key corresponds to a node's minimum key and each position covers the node's serialized bytes. 
This process of index derivation imposes two challenges in tuning problem.
First, node builders prefer their specific key-position patterns; however, their preference is often only known after applying them.
Furthermore, the next key-position collection may be easier or harder to be indexed, i.e. having different \emph{index complexities} (formalized in \cref{sec:system-building-selection}). To tackle both posterior preference and index complexity challenges, \oursearch explores different node builders (\cref{algo:main-tuning}, lines 3--6 and 8--9) and selects the best resulting layer for the given key-position collection (\cref{algo:main-tuning}, lines 11--12).


\begin{figure}[t]
  \centering
%   \vspace{2mm}
  \resizebox{0.9\linewidth}{!}{\input{figures/methodology/branch_bound}}
  \vspace{-2mm}
  \caption{\system automatic tuning algorithm, starting from the bottom (data layer) to the top. The label ``root'' indicates that the candidate should be the root layer with no further index layer, signifying the base case of the recursion. In this illustration, the algorithm selects $k = 3$ top candidates to branch out and finds candidates with $L = 1$ and $L = 2$ layers. \supawit{Make this into example}}
  \vspace{-3mm}
  \label{fig:branch_and_bound}
\end{figure}


% Branching out has an exponential complexity
Branching the exploration comes at a price: search time complexity may grow exponentially with respect to the data size. To limit the branching factor, \oursearch selects only the top-$k$ prospective candidates (\cref{sec:system-building-selection}) based on an upper bound of the index complexity (\cref{algo:main-tuning}, line 7). Our analysis (\cref{sec:system-analysis-complexity} shows that, in large range of $k$, \oursearch runs at a linear time complexity rather than the exponential one like the branching may suggest.

% When to stop building index layer
To complete the recursion base case, \oursearch must decide whether an additional index layer will be beneficial. \oursearch answers this question using an \emph{ideal index layer}: the best (possibly impossible) layer we can build on top. Specifically, an ideal index is the smallest index layer ($s(\Theta) = 1$ byte) with the finest precision ($\Delta(x; \Theta) = 1$ byte).
Thus, if the latency does not decrease with an ideal index layer, \oursearch can conclude safely that no more index layers can improve the overall lookup speed (\cref{algo:main-tuning}, lines 1--2).

% {
    % The overall building methodology \fixedRI{described in \cref{algo:main-tuning}} resembles SMA*.
    %     % across index layers. 
    % At each point in the optimization search graph, \system generates the next set of index layer candidates by
    %     combining node builders (\cref{sec:system-building-node-estimation}) 
    %         and a heuristic (\cref{sec:system-building-selection}) 
    %     to select the top-$k$ candidates to explore.
    % This process occurs recursively for each index layer in each branch,
    %     until it stops when \system determines
    %     no more indexes further built on top
    %         can improve the overall lookup latency,
    %     which is based on our \emph{ideal index layer}, as descried shortly.
        
    % % an ideal index could not possibly perform better than entirely fetching the latest layer, based on the storage profile. 
    
    % Unlike SMA*, however, \system implements a different form of heuristic
    %     to hard-bound the computational cost (or the number of nodes to visit).
    % That is, while SMA* can serve as a good framework for generic search problems,
    %     it is not ideal to apply directly to our setting
    %         because the default algorithm may explore an exponentially number of nodes,
    %     which is too expensive.
    % To tackle this, \system's heuristic (\cref{sec:system-building-selection})
    %     tightly upper-bounds the true cost (instead of lower-bounding in SMA*)
    %     to limit the number of nodes we have to explore
    % while providing a hard quality guarantee.
% }

% Similar to SMA*, \system evaluates each candidate using its current precision and future index complexity heuristic.
% However, \system heuristically prunes candidates instead of prioritizes them like in SMA*.
% As a result, \system is more computational efficient and easier to scale (\cref{sec:system-analysis-approx-factor}) than SMA* due to its exponential computation cost and decision dependency.
% Although this pruning may leave out the optimal candidate, \system's heuristic is an upper bound to the optimal solution, and so, \system can bound the risk between the heuristic value and the ideal index.

% {
    % \paragraph{Ideal Index Layer}
    
    % Our search process must answer a critical question: ``Should we (try to) stack one more layer on top?''
    % We answer this question with a notion of \emph{ideal index layer}.
    % An ideal index layer is the best possible layer we can build on top;
    %     thus, if the latency does not decrease with an ideal index layer,
    %         we can conclude that no more index layers can improve the overall lookup speed.
    % Specifically,
    % an ideal index is defined as the one 
    %     with the smallest index layer ($s(\Theta) = 1$ byte) and the finest precision ($\Delta(x; \Theta) = 1$ byte).
    % % Finally, after all branches converge and the best structure emerges, \system then persists the best index structure for the target data collection to storage.
% }


% \paragraph{Discussion}

% On the surface, \oursearch might resemble a simple grid search. We have experiment with many other optimization fashions including iterative searching and stream building, but in this case, simplicity wins with the following careful considerations.
% Like grid-search optimizations, \oursearch would have suffered from the curse of dimensionality. In index structure space, these hyperparameter dimensions refer to the number of layers $L$, node types, and node-specific hyperparameter. \system cures the curse in multiple ways.
% \system controls the grid resolutions and bounds (\cref{sec:system-building-node-estimation}) to find the optimal structure accurately up to an approximation factor (\cref{sec:system-analysis-approx-factor}) assuming some structure in the storage profile and node builders.
% According to our computation complexity analysis (\cref{sec:system-analysis-complexity}), \system balances the candidate branching factor with the anticipated index depth by selecting top-$k$ candidates (\cref{sec:system-building-selection}). In other words, if it expects a higher number of layers, it would prune the candidate more aggressively by selecting fewer $k$ candidates.
% \system's bottom-up tuning from data layer to root index layer naturally unfolds the storage model objective summation structure and localizes decisions on upper decision along with the recursion depth.
% With these corrections, \system can accelerate the tuning by parallelizing \oursearch along many axes such as data size and model diversity (\cref{sec:system-building-parallelism}), similarly to other grid search algorithms.

% At the core, candidate generation constructs multiple candidates in a bottom-up fashion, from lower to higher index layers. For a key-position collection to be indexed, \supawit{build next layer drafts using node builders (explain later), select top-$k$ drafts based on approximated complexity (explain later), generate new key-position collections for selected ones, recursively search for upper candidates, stack to make candidates, evaluate, and return best candidate} \supawit{stop criteria: when no ideal index could be faster} \supawit{MAYBE claim: adversarial exists for top-down construction}


% node fit here
\subsection{Node Builders}
\label{sec:system-building-node-estimation}
% node estimation: procedure to get parameters for the node from data
% node fitting: how well can the node fit with the data
% node development: process to create nodes, test them, and select the best node
% node building/construction (not really DS term): sounds like the process to come up with a node

A node builder turns the target key-position collection $D$ into an index layer $\Theta$. In other words, it is a function $F(D) = \Theta$ where $D = \left\{ (x_i, y_i) \right\}_{i=1}^n$ is a collection of keys $x_i$ together with their positions $y_i$, and $\Theta = \{ (z_j, \theta_j) \}_{j=1}^{n^{+}}$ is the index layer containing the per-node parameters $\theta_j$ with per-node key range $[z_j, z_{j+1})$. 
To build two types of nodes (\texttt{step} and \texttt{band}, sketched in \cref{fig:node_types}), 
    \system currently deploys three types of node builders below.
\begin{enumerate}[leftmargin=5mm,]
    \item \textbf{Greedy Step} (\texttt{GStep}$(p, \lambda_{GS})$) builds a $p$-piece step function with precision at most $\lambda_{GS}$ bytes. It iterates over each key-position pair $(x_i, y_i)$ and greedily determines whether to create the next constant function if $y^{+}_i - b_k > \lambda_{GS}$ where $(a_k, b_k)$ represents the current constant function. If so, the next constant function has a partition key $a_{k+1} = x_i$ and partition position $b_{k+1} = y_i$. Once it reaches $p$ pieces of constant functions, \texttt{GStep}$(p, \lambda_{GS})$ generates a $p$-piece \texttt{step} node.
    % and starts a new node.
    
    \item \textbf{Greedy Band} (\texttt{GBand}$(\lambda_{GB})$) builds linear band nodes by greedily fitting as many key-position pairs as possible,
        using a method called monotone chain convex hull~\cite{DBLP:journals/ipl/Andrew79ConvexHull},
        until we have $\Delta(x_i) > \lambda_{GB}$. 
    Then, 
    % When the precision is too coarse $\Delta(x_i) > \lambda_{GB}$, 
        it generates a \texttt{band} node with $(x_1, y_1, x_2, y_2, \delta)$. 
    % Rebuilding the linear function for each new key-position would be inefficient; instead, \texttt{GBand}$(\lambda_{GB})$ maintains a convex hull of key-position pairs included so far and queries the convex hull whether it can feasibly fit in a linear band function with a width $\delta \leq \lambda_{GB}$. 
    % This procedure is also known as the monotone chain convex hull~\cite{DBLP:journals/ipl/Andrew79ConvexHull}. 
    % In the total processing of 
    For $n$ key-position pairs, the convex hull inserts a key-position pair in $O(n)$ time ($O(1)$ amortized insertion) and answers a feasibility query in $O(n \log m)$ time ($O(\log m)$ amortized query) where $m$ is the average number of key-position pairs included in one linear band. Typically, $m$ is small when $\lambda_{GB}$ is small.
    
    \item \textbf{Equal Band} (\texttt{EBand}$(\lambda_{EB})$) builds linear band nodes by grouping key-position pairs in equal-size position ranges. That is, each group $\{(x_l, y_l)$, $(x_{l+1}, y_{l+1})$, $\dots,$ $(x_r, y_r)\}$ has a bounded position range $|y^{-}_l - y^{+}_r| \leq \lambda_{EB}$. It then fits a linear band function to each group and creates a \texttt{band} node. Note that the precision $\Delta(x_i)$ can vary depending on how ``linear'' the group is. \texttt{EBand}$(\lambda_{EB})$ groups by position ranges rather than key ranges so that the worst-case precision is controlled by $\lambda_{EB}$.
\end{enumerate}

\noindent
First, \texttt{GStep}$(p, \lambda_{GS})$ is equivalent to bulk indexing in a sparse B-tree with a fanout $p$ and page size $\lambda_{GS}$ bytes.
% where
% each intermediate sparse B-tree node has $p$ pointers 
%     with each pointer pointing to $\lambda_{GS}$ bytes of 
%     indexed data that may cover multiple B-tree nodes. 
Second, 
    \texttt{GBand}$(\lambda_{GB})$ is a generalization from step functions to linear functions with precision $\Delta(x_i) \leq \lambda_{GB}$.
Third, \texttt{EBand}$(\lambda_{EB})$ is another generalization focusing on the key-position group size $|y^{-}_l - y^{+}_r| \leq \lambda_{EB}$.


\input{figures/methodology/tuning_algorithm}


\paragraph{Granularity Exponentiation} $\lambda_{GS}$, $\lambda_{GB}$, and $\lambda_{EB}$ are called \textit{granularity},  which roughly control node builders' tendency to split key-position pairs apart. Because they correlate with the resulting node's precision $\Delta(x; \Theta)$, \system needs to determine the appropriate granularity for each node type.

\system creates many candidate node builders $\calF$ by sampling the granularity on an exponential grid: $\lambda_{low}, \lambda_{low} (1 + \epsilon), \lambda_{low} (1 + \epsilon)^2, \dots \lambda_{high}$ where $(\lambda_{low}, \lambda_{high})$ are the bounds and $\epsilon > 0$ controls the exponentiation base. Smaller $\epsilon$ implies a finer search which improves optimization accuracy but increases tuning time. For example, if we set $\lambda_{low} = 2^6$, $\lambda_{high} = 2^{20}$, and $1 + \epsilon = 2$ with $p = 16$, then 
% the candidate node builders 
$\calF$ contains 45 builders in total:
\begin{equation}
\begin{split}
\calF
    =& \{\texttt{GStep}(16, 2^6), \texttt{GStep}(16, 2^7), \dots, \texttt{GStep}(16, 2^{20})\} \\
    &\cup \{\texttt{GBand}(2^6), \texttt{GBand}(2^7), \dots, \texttt{GBand}(2^{20})\} \\
    &\cup \{\texttt{EBand}(2^6), \texttt{EBand}(2^7), \dots, \texttt{EBand}(2^{20})\}
\end{split}
\end{equation}


\subsection{Top-k Candidates by Index Complexity}
\label{sec:system-building-selection}

\input{figures/methodology/index_complexity}

Before branching out, \system selects only top-$k$ candidates with the highest potential to be in the optimal design. Suppose there exists an oracle that minimizes the objective function on a key-position collection $D$ under the storage profile. We call the optimal search cost under storage profile $T$: \textit{index complexity} $\tau(D; T)$. If $\tau(D; T)$ is known, selection of candidates $\calC = \{(\Theta_i, D_i)\}_{i=1}^{|\calF|}$ would be as straightforward as \cref{eq:selection-oracle}. That is, we could simply select the top-1 candidate and avoid branching out.
\begin{equation} \label{eq:selection-oracle}
    (\Theta^{*}, D^{*}) = \argmin_{(\Theta_i, D_i) \in \calC} \tau(D_i) + \E_{x \sim \calX} \left[ T(\Delta(x; \Theta_i)) \right]
\end{equation}

Unfortunately, $\tau(D; T)$ is unknown for a large class of indexes supported by \system. Instead, \system uses a surrogate upper bound to the index complexity: \textit{step index complexity} $\hat{\tau}(D; T) \geq \tau(D; T)$. Specifically, $\hat{\tau}(D; T)$ imitates a step-function hierarchical index that partitions the key-position collection $D$ into groups with arbitrary position ranges. Let $s_D = y^{+}_{|D|} - y^{-}_1$ be the total size of the candidate layer, $\hat{\tau}(D; T)$ tries to build ideal step indexes with different numbers of layers $L \in \{0, 1, \dots, O(\log s_D)\}$. For each $L$, it perfectly balances both root layer size and subsequent precisions 
so that $s(\Theta_L) = \Delta(x; \Theta_l) = \sqrt[L+1]{s_D s_{step}^{L}}$.
% (\cref{eq:selection-step-balance}).
This 
% takes into account of 
considers the total size $s_D$ and the ideal size for each 1-piece step node $s_{step}$ (e.g., 16 bytes for 8-byte key and position types). 
% \begin{equation} \label{eq:selection-step-balance}
%     % s(\Theta_L) \approx \Delta(x; \Theta_l) = s_D^{1 / (L + 1)} s_{step}^{L / (L + 1)} \qquad, l \in \{1, \dots, L\}
%     s(\Theta_L) \approx \Delta(x; \Theta_l) = \sqrt[L+1]{s_D s_{step}^{L}} \qquad \text{for } l \in \{1, \dots, L\}
% \end{equation}
% (data_size as f64).powf(1.0 / (num_layers + 1) as f64)
%                   * (STEP_SIZE as f64).powf(num_layers as f64 / (num_layers + 1) as f64);
Lastly, $\hat{\tau}(D; T)$ then outputs the lowest storage model cost as the step index complexity (\cref{eq:selection-step-complexity}).
\begin{equation} \label{eq:selection-step-complexity}
    % s(\Theta_L) \approx \Delta(x; \Theta_l) = s_D^{1 / (L + 1)} s_{step}^{L / (L + 1)} \qquad, l \in \{1, \dots, L\}
    \hat{\tau}(D; T) = \min_{L \in \{0, 1, \dots, O(\log s_D)\}} (L + 1) \times T \left( \sqrt[L+1]{s_D s_{step}^{L}} \right)
\end{equation}

Note that $\hat{\tau}(D; T)$ is only interested in the integer $s_D$ (not the distribution of $D$);
    thus, $\hat{\tau}(D; T)$ can be arithmetically computed (hence cheap). 
    % and all calculations are arithmetic; 
\cref{fig:index-complex} shows the general shape of $\hat{\tau}(D; T)$ with respect to the collection size $s_D$, under an affine storage profile $T$. Notice the sudden index complexity cliffs (such as those around $s_D = 1$MB in \cref{fig:index-complex-latency}), marking the boundaries between different chosen numbers of layers in \cref{eq:selection-step-complexity}. The technique to minimize an objective based on its cheaper upper bound is related to majorize-minimization algorithms~\cite{DBLP:books/daglib/Lange2016MMalgorithms}.

\subsection{Parallel Tuning}
\label{sec:system-building-parallelism}

\system is highly parallelizable from three sources of parallelisms as described below, 
    ordered from finest to coarsest layers. 
It is worth noting that, with a proper branching (\cref{sec:system-analysis-complexity}), 
    the node-building step is the primary target for parallelization.
    % in the building procedure 
% and is the main target for parallelization.

\paragraph{From Data Partitioning} \system partitions the key-position collections, uses a node builder to build sub-range candidates, and merges them into a candidate. 
This is possible because \system's existing node builders generate a piecewise function that can be merged together across different key ranges. 
By default, \system breaks a key-position collection into partitions, each containing 1 million key-position pairs. 
Thus, \system can scale with growing data sizes 
    by increasing the level of parallelisms accordingly.

\paragraph{From Node Builders} 
Although \cref{algo:main-tuning} calls node builders in loops, the invocations are independent of one another. 
\system conveniently turns the for-loop into a parallel mapping to produce $(\Theta_{\text{next}}, D_{\text{next}})$ and collecting into the candidate set $\calC$. With more parallelisms, \system can then scale along with the diversity of node builders to capture wider key-position patterns.

One may consider iterative building alternatives that choose the next node builder setting based on past iterations. However, they will process through the key-position collection as many rounds as the number of iterations. In contrast, given enough parallelism, \system can generate multiple candidates using the same time as generating one candidate, equivalent to processing the key-position collection in one round. Since \system aims to handle a large data layer, processing in many rounds is slow and undesirable.

\paragraph{From Branching} 
\system can recursively call \cref{algo:main-tuning} in parallel and select the best index structure with the minimum storage model cost. This source of parallelism allows \system to explore more candidate branches and especially higher structures when favored by the storage profile (e.g., low bandwidth and low latency).


\subsection{Analysis}
\label{sec:system-analysis}

Branching recursive optimization requires a balancing between the branching factor and depth. If \oursearch branches out to too many candidates relative to the index depth, it would become uncontrollably slow. On the other extreme, it could miss the optimal candidate branch. We first analyze the tuning time complexity with respect to a choice of hyperparameter. Then, we attempt to provide an approximation factor of the automatic tuning. 
% \todo{difference from SMA* by upperbound --> faster, why it's ok?}

% \paragraph{Time Complexity}

\begin{theorem} \label{sec:system-analysis-complexity}
\textit{Time complexity}: Let there be $n$ key-position pairs, $L$ layers to be explored at most according to the storage profile $T$, and $|\calF|$ node builders. If \oursearch selects at most $k \leq \sqrt[L+1\;]{n}$ candidates then the time complexity is at most $O((L + 1) |\calF| n)$.
\end{theorem}

\begin{proof}
Suppose the data $D$ consist of $n$ key-position pairs with total data size $s_D$. Let $L$ be the maximum number of layers expected to be explored, which has the upper bound $L_{\max} \geq L$: the number of layers chosen by the step index complexity (\cref{eq:selection-step-complexity}).


\input{figures/experiments/I_latency_cold}
% \input{figures/experiments/I_latency_curve}


Because our node builders all process a $O(n)$ key-position collection in $O(n)$ time, the time to build all $|\calF|$ candidates is $O(|\calF| n)$. Next, considering the worst case compression ratio $O(n^{\frac{1}{L + 1}})$ and the number of branches $k$, we expect $O(n^{\frac{L}{L + 1}})$ key-position pairs and so the time complexity in the next layer is $O(|\calF| k n^{\frac{L}{L + 1}})$. The branching and compression of key-position pairs continue until the root layer. In summary, the total time complexity in $L$-layer branching recursion is as followed whose last step is the closed-form formula to the geometric series.
\begin{equation} \label{eq:system-time-complexity-full}
O\left(|\calF| \sum_{l=0}^{L} k^l n^{\frac{L + 1 - l}{L + 1}}\right)
    % = O\left(|\calF| \frac{n^{\frac{1}{L+1}}\left(n-k^{\left(L+1\right)}\right)}{\left(n^{\frac{1}{L+1}}-k\right)} \right)
    = O\left(|\calF| n \frac{1 - k^{L+1} / n}{1 - k / n^{\frac{1}{L+1}}} \right)
\end{equation}

Under $k^{L+1} / n \leq 1$ (i.e. $k \leq \sqrt[L+1\;]{n}$), this reduces to $O(|\calF| (L + 1) n)$ when $n \rightarrow \infty$.
\end{proof}


% P: Build time \& space complexities (3 node fitting methods, step complexity, total build, with parallelism)

% $$O(n + k n^{L_{\max} / (L_{\max} + 1)} + k^2 n^{(L_{\max} - 1) / (L_{\max} + 1)})$$

% $$O\left(\sum_{l=0}^{L_{\max}} k^l n^{\frac{L_{\max} + 1 - l}{L_{\max} + 1}}\right) = O\left( \frac{n^{\frac{1}{L+1}}\left(n-k^{\left(L+1\right)}\right)}{\left(n^{\frac{1}{L+1}}-k\right)} \right)$$

% which is asymptotically linear in data size $O(n)$ (\url{https://www.desmos.com/calculator/hpfughrx5g}, \url{https://www.desmos.com/calculator/fmfzdoehlc}), but if $k^{L+1} \geq n$ or $L \geq \log_k(n) - 1$ then $O(k^L)$ (\url{https://www.desmos.com/calculator/zxb7nygi49}. At balance point $\left(L_{max}+1\right)k^{\left(L_{max}+1\right)} = (L + 1) n$ \url{https://www.desmos.com/calculator/zum03kegvu}

% Via Master's theorem~\cite{??}

% \begin{theorem}
% \label{sec:system-analysis-approx-factor}
% \textit{Approximation factor}: Under step complexity $\tau_{step}$, for each of the three nodes, exponentiation with parameter $1 + \epsilon$ gives $(1 + \epsilon)$-approximation of the optimal structure.
% \end{theorem}

% \begin{itemize}
%     \item Step complexity upper-bounds the complexity: $\tau_{step} \geq \tau$
%     \item Monotonicity: As $\lambda$ increases, the step complexity decreases and precision is coarser. For $\lambda_{i+1} = (1 + \epsilon) \lambda_i$, $\tau_{step}(\lambda_i) \geq \tau_{step}(\lambda_{i+1})$ and $\Delta(\lambda_i) \leq \Delta(\lambda_{i+1})$
%     \item Say the optimal $\lambda^{*} = \argmin_\lambda \tau_{step}(\lambda) + T(\Delta(\lambda))$ is in $[\lambda_i, \lambda_{i+1}]$
%     \item By monotonicities, $\tau_{step}(\lambda^{*}) + T(\Delta(\lambda^{*})) \geq \tau_{step}(\lambda_{i+1}) + T(\Delta(\lambda^{*}))$
%     \item By monotonicities, $\tau_{step}(\lambda^{*}) + T(\Delta(\lambda^{*})) \geq \tau_{step}(\lambda^{*}) + T(\Delta(\lambda_i))$
%     \item By monotonicities, $\tau_{step}(\lambda^{*}) + T(\Delta(\lambda^{*})) \geq \tau_{step}(\lambda_{i+1}) + T(\Delta(\lambda_i))$
%     \item \tofix{Lacking}: $T(\Delta(\lambda_i)) \geq \alpha T(\Delta(\lambda_{i+1}))$ (possible?) or $\tau_{step}(\lambda_{i+1}) \geq \alpha \tau_{step}(\lambda_i)$ (likely false)
% \end{itemize}

% \paragraph{Bottom-up and Top-down equivalence}
% \label{sec:system-analysis-bottomup-topdown}

% \paragraph{Node type preference}

% P: Best and worst cases for each node type

% P: [Adversarial for top-down or equivalence] given a top-down index building approach that partition data into groups using $O(1)$-sized function, prove that there exists a data such that at least one group is skewed

% \paragraph{Differences from PGM-index}

% Q: What are differences between ERMI and PGM-index?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Other Implementation Details}
\label{sec:system-implement}

We implement \system in Rust~\cite{airindex_repo}~\footnote{https://github.com/\githuborg/airindex-public}.
Like many data systems, it has two explicit levels in its memory hierarchy: 
    the underlying storage and its internal read-through cache. 
\system interacts with storage through an abstract interface, in which concrete implementations serve partial range reads at their best effort. 
Currently, \system's internal zero-copy read-through cache employs a first-in-first-out (FIFO) eviction policy due to its admission simplicity.
% and the abundance of cache space in our experiment settings.
Apart from customized node type format, \system serializes the metadata together with root layer as a byte array in the Postcard~\cite{postcard} format via Serde~\cite{serde}. 
% During a restart, \system reads this metadata-root
% in its internal cache prior to \cref{algo:query-process}.

% \paragraph{Physical Layer and Node Format}

% \supawit{Byte representations of each node type \& layer format. How we organize blocks and pages. How this helps with error correction.}

% \paragraph{Metadata}
% \label{sec:system-implement-metadata}

% \supawit{Root layer trick, Postcard serialization}

% \paragraph{Memory Hierarchy and Interface}

% \supawit{Our implementation works from file system. Cache hierarchy (NFS, OS, memory mapping). Describe how it Fetch, bounded prefetch. Other platform (aws, gcp)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Extension Opportunities}
% \label{sec:system-extensions}

% \paragraph{Data Mutability}
% % Even though \system currently tunes for immutable indexes, these immutable indexes 
% \system can be extended to enable
% % the application's mutable data
% efficient data updates in three ways. 
% %
% % 1) \system can tune an initial version of an updatable index, and let the application follow updatable index procedures. 
% 1) \system can follow the \alex's existing update procedures,
%     while \system's optimization serves as the design recommendation
% for initial bulk loading.
% % For example, \system can act as a bulk loading of \alex, with awareness of data and storage. 
% %
% 2) 
% % We can readjust position from bytes to larger granularity, so data mutations trigger index re-tuning less often.
% Instead of modeling every key position, we can model key positions
%     at the page level, requiring lesser tuning.
% %
% 3) The application can buffer writes to defer index building until write batches are large enough. 
% For example, \system can tune learned indexes for higher layers in LSM-trees~\cite{DBLP:journals/acta/ONeilCGO96LSMTree}, possibly following lessons from~\cite{DaiXGAKAA2020BourbonLSM}. 

% \paragraph{Continuous Redesigning}
% While \system suggests an optimal index design,
%     as the dataset updates (e.g., inserts/deletes)
% and the storage performance changes over time,
% the initial index design may no longer be optimal,
%     expecting potential performance improvements
% with gradual index redesigning.
% There are three types of gradual redesign opportunities:
% 1) using a different model type for a layer,
% 2) creating a new root layer if that can reduce the overall latency,
% and 
% 3) remove the root if larger cache becomes available
%     or enough records have been removed from a dataset.
% These decisions can still be made in a principled way
%     using \cref{eq:emm-totalcost}
% and in an efficient way
%     employing our top-$k$ search mechanism (\cref{sec:system-building-selection}).
% Beyond data mutability, we may desire to tune mutable indexes. If we can characterize mutable operations (e.g., expected distribution), minor modifications to \system may suffice: expanding target class of indexes (\cref{sec:system-overall-class-of-index}), including writing into query process (\cref{sec:querying}), adding writing costs to the objective function (\cref{sec:objective}), and possibly prepare the tuning algorithm to expect index structural changes (\cref{sec:system-building-overall}).

% Otherwise, if mutable operations cannot be characterized (for example, due to unpredictability, strict requirements, or other reasons), offline tuning algorithms like \system would be unsuitable and need a major redesign. We may integrate a mutable index with a ``tuning'' logic to restructure the index during mutation based on a storage-aware cost model similar to \cref{eq:emm-totalcost}. Alternatively, in the spirit of \system's candidate branching, we may maintain top-$k$ mutable indexes with different designs to compete to be the ``active'' index. These online tuning mechanisms should identify many practical aspects such as operability, distribution shift, adversary, and performance guarantees.

% \paragraph{Cache Awareness}
% To find optimal indexes 
% in consideration of the size of local cache,
% % to a fixed cache capacity, 
% we can easily modify \system to search for indexes whose root layer fits in the cache. 
% Specifically, the tuning algorithm (\cref{algo:main-tuning}) can stop when a layer fits within the cache, and the objective (\cref{eq:emm-obj-airindex}) will substitute $T(s(\Theta_L))$ terms with a cache read cost. 
% % We defer the study of this modification in the future 
% % due to technical difficulties in standardizing cache allowance among baselines.
% %
% For large cache capacity (i.e. linear with respect to data size) or highly skewed query keys, one should consider directly caching the key-value pairs in order of their popularity and let the residual cache store the root layer like the earlier case. One should study how to allocate the residual and how to characterize the query distribution more cautiously.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\fixed{
\section{Extensions}
\label{sec:discussion}

\paragraph{Supporting Updates}
Although \system does not optimize for write workloads, it can tune and build an index that supports write operations. For example, \system can serves as the initial bulk loading of an updatable index (e.g. \alex). However, the updatable index may evolve suboptimally. To reduce the frequency of structural index updates, we can enlarge the position granularity from bytes to pages, or we can buffer writes similarly to LSM-trees~\cite{DBLP:journals/acta/ONeilCGO96LSMTree}, possibly following lessons from~\cite{DaiXGAKAA2020BourbonLSM}.

\paragraph{Cache-aware Optimization}
\system can tune an index to a cache hierarchy by directly optimizing on the original cost (\cref{eq:original-cost}) with further specifications on the distribution of cache hit $C_l$ and the cost of cache access $\calL_{\text{cache}}$. This modification then only affects the index complexity $\hat{\tau}$ and candidate selection in \oursearch.
While this work does not include explicit results for cache-aware optimization, \cref{fig:I_latency_curve} indicates that the indexes built with cache-pessimistic optimization already offer high performance than other existing methods across a wide range of cache warmness.
}

% theoretical, hint: saturation

==> sections/old_motivation.tex <==
\input{figures/background/structures}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivation}
\label{sec:bg}

This section describes the limitations in the existing work
    and explain how we find an optimal index design.
        % that can directly minimizes the end-to-end latency.
    % in a principled way.

\paragraph{Learned Indexes}
\label{sec:bg-indexes}

Learned indexes~\cite{Kraska2018} 
    connects indexing and the density estimation problem
by equating an index to a model 
    expressing a cumulative density function (CDF) of sorted data.
Since then, learned indexes
% (a.k.a. CDF-based indexes) 
% have found applications in complex datasets and 
has been extended 
    to handle mutability~\cite{DBLP:journals/pvldb/FerraginaV20PGMIndex, DingMYWDLZCGKLK2020ALEX, DBLP:conf/sigmod/Li0ZY02020LISA},
multi-dimensional datasets~\cite{DBLP:journals/pvldb/DingNAK2020Tsunami, DBLP:conf/vldb/0001KH20/Hadian2020HandsOff},
etc.
% as well as dynamic data layout.  
% For example,  manages multi-dimensional datasets, \cite{DBLP:journals/pvldb/FerraginaV20PGMIndex,DingMYWDLZCGKLK2020ALEX} enable provably efficient index updates, \cite{DBLP:conf/vldb/0001KH20/Hadian2020HandsOff} designs both multi-dimensional and mutable learned index, and \cite{DBLP:conf/sigmod/Li0ZY02020LISA} proposes a mutable learned index for a multi-dimensional dataset with a dynamic data layout. 
For more in-depth study of the taxonomy, please see \cite{AlMamun2020TutorialLearnedIndexes}.

\paragraph{Limitations}
First,
existing learned indexes optimize for size and accuracy metrics,
which may not always be strongly correlated with the end-to-end lookup latency,
% rather than directly performance metrics. Despite their superficial relation, the two sides may be uncorrelated, for example, 
as demonstrated by 
the U-shape curves between learned index size and lookup time presented in \cite{DBLP:journals/pvldb/MarcusKRSMK0K20BenchmarkLearned}. 
Second, 
while replacing existing B-tree nodes with learned functions
    is a promising direction,
finding optimal learned functions
    in a large search space may not be computationally tractable;
for that reason, existing methods use the same type of models for the
    entire index, instead of tuning each layer.
% like other machine learning applications, learned indexes risk suboptimal designs due to a wider variety of design choices: the family of functions, parameter estimation, objective formulation, etc.

% \supawit{Accuracy is not all of latency} \supawit{Fast learned index needs careful design} \supawit{Limited works on external storage}


\subsection{Goal \& Challenges}
\label{sec:bg-problem}

We aim
% We pursue a straightforward goal: 
to find an index structure 
% on a given dataset 
that minimizes the end-to-end lookup latency
    for a given dataset and storage. 
This task involves the three types of challenges as follows.
% To do so, our solution must overcome these challenges.

\paragraph{Storage Diversity} Storages are diverse; each behaves differently depending on its hardware/software designs. 
To correctly reflect their impact on lookup latencies,
% Because the underlying storage 
% % determines 
% impacts
% the lookup latency, an appropriate 
our objective must allow a generic storage abstraction
    such that the abstraction can be well incorporated in our optimization
while it represents realistic performance.
% a generic storage abstraction is required to construct a generic and meaningful objective. 
% Extremely realistic storage model may introduce unnecessary complexity preventing a tuning algorithm to progress; conversely, a simplistic storage model may suggest an attainable optimizer but practically suboptimal. Our solution must select a sufficiently simple storage abstraction to formulate a solvable objective while keeping a suitable level of realism.

\paragraph{Possibilities of Indexes} 
% The invention 
The notion of learned indexes 
    encompasses a large number of design choices,
which also means
% has led to an explosion of the set of possible indexes. This lends us a powerful tool to handle ever-growing data diversity, but also a double-edged sword in our problem of interest: 
a larger search domain, often implying harder optimization. 
Our solution must realize the structure of learned indexes and leverage computation resources to efficiently guide the optimization in the exponentially large set of possibilities.

% \paragraph{Interdependency} Beyond the sheer size of search space, the constraint describing all valid indexes is nonetheless intricate. A change in a parameter of the index must preserve the ability to answer queries correctly. Almost always, such a change propagates into changes in parameters downwards (e.g., top-down index) and/or upwards (e.g., bottom-up index). 
% Our solution must disentangle this interdependency to efficiently find the desired structure.


\paragraph{Fine-grained Optimization}

Different models prefer different data patterns. 
To avoid suboptimal indexes, 
our solution needs to select models according to 
    the data patterns at an index sub-structure level 
    such as block-wise, layer-wise, or node-wise.
% In hindsight, 
\system's 
% auto-tuning algorithm 
fine-grained per-layer optimization
leverages this opportunity.
% has shown benefits in per-layer optimization. 
For example, in the \texttt{gmm} dataset from the experiments stored on a SSD, \system recommends an index with a step-function root layer (similar to B-Tree layers) followed by a piecewise-linear (PWL) layer (\cref{fig:structures:system}), which achieves 28\% speedup over a tuned B-Tree (\cref{fig:structures:btree}), 18\% speed up over a PWL index with the same precision as the tuned B-Tree (\cref{fig:structures:band}), and 7\% speedup over a tuned PWL index (\cref{fig:structures:tuned-band}).

\subsection{Our Approach}
\label{sec:bg-approach}

% The key to our optimization method is \emph{\supawit{KEY IDEA}}
    % \emph{the ability to consider exponentially many sets of index design parameters in an extremely efficient way using an accurate predictor that can guide us toward optimal design parameters.}

To tackle these challenges, \system generalizes storage performance using a profile function $T(\Delta)$ representing the time to read $\Delta$ bytes from the storage. Furthermore, \system formally defines a target class of indexes that contains a large set of learned indexes yet provides a precise query process. Building upon this storage profile and class of indexes, \system formulates an objective decomposable into a sequence of index-building decisions that ``compress'' a dataset into a smaller dataset (called index layer) and recursively shrinks the tuning problem at each step. The decomposition allows \system to manage data-model preference layer by layer.

Inspired by a generic graph search algorithm called Simplified Memory Bounded A* (SMA*)~\cite{russel1992effcient}, \system's index tuning views the index building decisions as a graph search problem where edges represent decisions while each vertex represents an index layer associated with a lookup latency cost. SMA* is a shortest path algorithm for graphs whose number of reachable vertices overwhelm available memory. To work with the tight budget, it relies on a domain-specific heuristic to select a few candidate vertices. SMA* works well when the optimal vertex is near the starting point. Similarly to SMA*, \system's tuning algorithm navigates the exponentially large reachable index-building combinations by relying on a \emph{index complexity} heuristic. Moreover, by nature of SMA* exploration and index building, \system is able to exploit parallelism to accelerate the tuning to be comparable to simply an index building. Thanks to the compression power of learned indexes pulling the optimal index closer, \system's versatile index tuning can find a fast index tailored for the underlying data and storage.



% Learning-based methods have been reshaping the index design methodology
%     by delivering significantly faster lookup speed
%     with the layers/nodes fitted to data.
% The state-of-the-art
%     includes (i) sophisticated models 
%         that can represent complex data
%             (e.g., RMI~\cite{kipf2018learned}, RadixSpline~\cite{DBLP:conf/sigmod/KipfMRSKK020RadixSpline}, PGM-Index~\cite{DBLP:journals/pvldb/FerraginaV20PGMIndex}),
%     (ii) updatable models for supporting insertions/deletions (e.g., ALEX~\cite{DingMYWDLZCGKLK2020ALEX}),
%     (iii) training over unordered datasets (e.g., LSI~\cite{kipf2022lsi}),
%     etc.
% Compared to B-trees~\cite{Bayer1972,Comer1979, Graefe2001, Chen2001, Chen2002, Wang2020, Wu2010, Zhou2014, Bin2014, bender2000CacheObliviousBtree},
%     these methods produce hierarchical indexes with \emph{succinct nodes} by learning 
%     from specific data distributions;
%     using succinct nodes,
%         a lookup process can traverse an index more quickly,
%     needing to fetch fewer bytes from storage.


% Learning indexes from specific data distributions is a great start 
%     toward designing high-performance indexes;
% however, we observe a significant missed opportunity in existing approaches.
% That is,
%     % we recognize significant a missing opportunity.
% % That is,  that 
% \emph{their optimization does not consider
%     the actual data fetch time as a first-class citizen}.
%         % the actual time needed to fetch data
%         %     from a storage layer (e.g., SSD, NFS)}.
% Accordingly,
%     the indexes learned \emph{only} from data distributions may 
%         deliver poorer performance compared to
%     indexes learned from storage performance as well as data.
% Our recent work~\cite{supawit2022airindex}
%     shows the viability of this idea---\emph{learning indexes
%         from both data distributions and storage performance}---by
%     sharing preliminary results obtained with a heuristic index builder;
% however, such heuristic approaches cannot generalize to
%     different datasets and storage
%         to offer optimal performance in various settings.
